Magnification Prior: A Self-Supervised Method for Learning Representations on Breast Cancer Histopathological Images

This work presents a novel self-supervised pre-training method to learn efficient representations without labels on histopathology medical images utilizing magnification factors. Other state-of-theart works mainly focus on fully supervised learning approaches that rely heavily on human annotations. However, the scarcity of labeled and unlabeled data is a long-standing challenge in histopathology. Currently, representation learning without labels remains unexplored for the histopathology domain. The proposed method, Magnification Prior Contrastive Similarity (MPCS), enables self-supervised learning of representations without labels on small-scale breast cancer dataset BreakHis by exploiting magnification factor, inductive transfer, and reducing human prior. The proposed method matches fully supervised learning state-of-the-art performance in malignancy classification when only 20% of labels are used in fine-tuning and outperform previous works in fully supervised learning settings. It formulates a hypothesis and provides empirical evidence to support that reducing human-prior leads to efficient representation learning in self-supervision. The implementation of this work is available online on GitHub - https://github.com/prakashchhipa/Magnification-Prior-Self-Supervised-Method

==> WACV 2021-MPCS_Arxiv/sections/0_abstract.tex <==
% Analysis of histopathological images to diagnose cancer has been active field of research in computer vision.
% Given huge variability in appearance of tissues, images are acquired on different optical magnifications which imposes challenges in learning the representations.
% Further, the scarcity of such data, specifically annotated data makes it more challenging to obtain state-of-the-art performance.
% In this paper, we propose novel self-supervised methods to learn efficient representations without need of labels.
% Proposed methods formulates contrastive similarity by exploiting magnification prior and inductive transfer which enable to learn representations on small-scale dataset and attempts to reduce human prior.
% We evaluate all the variants of the proposed method on BreakHis breast cancer dataset for the downstream task of malignancy classification by obtaining more robust experimentation protocol.
% The proposed methods obtains state-of-the-art performance in limited labeled data setting when using only $20\%$ labeled data and outperforms previous benchmarks extensively in fully supervised fine-tuning.
% Finally, we also investigate inter-magnification performance of proposed methods and preform underlying analysis.
% The implementation of this work is available online on github\footnote{\url{https://github.com/prakashchhipa/Magnification-Prior-Self-Supervised-Method}}.

\begin{comment}
\todo Rewrite
%- Abstract new attempt

Analysis of histopathological images to diagnose cancer has been an active field of research in computer vision.
Given huge variability in the appearance of tissues, images are acquired on different optical magnifications, which imposes challenges in learning image representations.
Further, the scarcity of such data, specifically annotated data, makes it more challenging to obtain state-of-the-art performance.
This paper proposes a novel self-supervised method, Magnification Prior Contrastive Similarity (MPCS) to learn efficient representations without labels.
The proposed method formulates contrastive similarity by exploiting magnification prior and inductive transfer, enabling learning representations on small-scale datasets and reducing human prior. 
This work evaluates all the variants of the proposed method on three public datasets of breast cancer including the BreakHis~\cite{spanhol2016dataset}  dataset for the downstream task of malignancy classification by obtaining a more robust experimentation protocol.
%The proposed methods obtain state-of-the-art performance in limited labeled data settings when using only $20\%$ labeled data and outperform previous benchmarks extensively using fully supervised fine-tuning.
The proposed method obtains state-of-the-art performance on the dataset and is competitive with previous work even when only 20\% of the labeled data is used.
Finally, this work proposes a hypothesis for how human priors can affect the performance of self-supervised models, which requires further investigation.
%Finally, this work investigates the cross-magnification performance of proposed methods and performs an underlying analysis.

\end{comment}




%1. topic sentence (1)
%2. Sota (1)
%3. shortcomings (1-2)
%4. contrib (1-3)
%5. results (1)
%6 further implications (0-1)

This work presents a novel self-supervised pre-training method to learn efficient representations without labels on histopathology medical images utilizing magnification factors.
Other state-of-the-art works mainly focus on fully supervised learning approaches that rely heavily on human annotations.
However, the scarcity of labeled and unlabeled data is a long-standing challenge in histopathology. Currently, representation learning without labels remains unexplored in the histopathology domain.
The proposed method, Magnification Prior Contrastive Similarity (MPCS), enables self-supervised learning of representations without labels on small-scale breast cancer dataset BreakHis by exploiting magnification factor, inductive transfer, and reducing human prior.
The proposed method matches fully supervised learning state-of-the-art performance in malignancy classification when only 20\% of labels are used in fine-tuning and outperform previous works in fully supervised learning settings for three public breast cancer datasets, including BreakHis. Further, It provides initial support for a hypothesis that reducing human-prior leads to efficient representation learning in self-supervision, which will need further investigation.
The implementation of this work is made available online on GitHub\footnote{\scriptsize{\url{https://github.com/prakashchhipa/Magnification-Prior-Self-Supervised-Method}}}.

\textit{Keywords: self-supervised learning, contrastive learning,  representation learning, breast cancer, histopathological images, transfer learning, medical images}

==> WACV 2021-MPCS_Arxiv/sections/1_introduction.tex <==
% \begin{figure}[h]
%     %\centering
%     \includegraphics[width =\linewidth]{sections/figures/fig_BreakHis_intro.png}
%     \caption{A slide of malignant tumor of BreakHis dataset seen in different magnification: (a) 40X, (b) 100X, (c) 200X, and (d) 400X}
%     \label{fig:fig_breakHis_intro}
% \end{figure}

\begin{comment}


\begin{figure}
\centering
\begin{subfigure}{.49\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{sections/figures/40X.JPG}  
  \caption{}
%   \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.49\columnwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{sections/figures/100X.JPG}  
  \caption{}
%   \label{fig:sub-second}
\end{subfigure}
\newline
\begin{subfigure}{.49\columnwidth}
  \centering
  % include third image
  \includegraphics[width=\linewidth]{sections/figures/200X.JPG}  
  \caption{}
%   \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}{.49\columnwidth}
  \centering
  % include fourth image
  \includegraphics[width=\linewidth]{sections/figures/400X.JPG}  
  \caption{}
%   \label{fig:sub-fourth}
\end{subfigure}
\caption{A slide of malignant tumor of BreakHis dataset seen in different magnification: (a) 40X, (b) 100X, (c) 200X, and (d) 400X}
\label{fig:fig_breakHis_intro}
\end{figure}

\end{comment}

\begin{figure}[!ht]
    \centering
    \includegraphics[width =\linewidth]{sections/figures/mpcs_intro.png}
    \vspace{-0.6cm}
    \caption{The proposed approach comprises three steps: (1)~Parameters initialization with supervised ImageNet weights. (2)~Self-supervised pre-training on unlabeled BreakHis histopathology images using proposed method \textbf{Magnification Prior Contrastive Similarity} to provide positive pairs by exploiting supervision signal, e.g., magnification from data and reducing human prior. (3) Fine-tuning on histopathology images for the downstream task.}
    \label{fig:mpcs_intro}
    \vspace{-6mm}
\end{figure}

\begin{comment}

Automated detection of cancerous tissue from images has been an active research field for several decades~\cite{suzuki1992development}.
Machine learning has been a powerful tool, and in the last decade, deep learning has enabled great strides in the field~\cite{komura2018machine}.
Cancer diagnosis by analyzing histopathological images is established as a very challenging task in computer vision.
Given huge variability in the appearance of tissues, images are acquired on different optical magnifications, which imposes troubles in learning the representations.
Further, the scarcity of such data, specially annotated data, makes it more challenging to obtain state-of-the-art performance.

This work investigates label efficient representation learning and proposes a novel self-supervised method, Magnification Prior Contrastive Similarity (MPCS), to learn efficient representations of unlabeled histopathological images. 
The proposed method formulates contrastive similarity by exploiting magnification prior and inductive transfer, enabling learning representations on small-scale datasets. 
Further, learned representations are exploited to accomplish the tasks of malignancy classification. A complete approach is depicted in Figure~\ref{fig:mpcs_intro} 

%This work evaluates all the variants of the proposed method on BreakHis\cite{spanhol2016dataset} breast cancer dataset for the downstream task of malignancy classification in a limited labeled data setting using only 20\% labels. Also, fully supervised learning using all labels in the train set by obtaining a more robust experimentation protocol. 
Following are the main contributions of the work:
\end{comment}


%Introduction: topic sentence is histopathology image analysis
Cancer diagnosis by analyzing histopathological whole-slide images (WSI) is an active research field in machine learning~\cite{komura2018machine}.
%Until now, analysis of histopathological samples by visual inspection under microscopy at different magnifications is most widely used method.
%Currently, the most widely used method for analysis of histopathological samples is visual inspection under microscopy at different magnification.
%Visual inspection follows a pyramid structure where smaller magnification present structural information of tissues and high magnification captures cellular details.
%The visual inspection follows an pyramid approach where structural information is viewed at low magnification and cellular details captured at high magnification.
%Results made by pathologist are based on both types of details but greatly affected by stain mechanism being used.
%Using automated classification of histopathological WSI might make cancer diagnosis faster and less prone to error.
%Automated classification of histopathological WSI can make cancer diagnosis faster and less prone to error.


%Background (to generate demand for purpose) - Topic sentence around data scarcity in all sense
%The main challenge for most explored supervised learning approaches for classification of histopathological WSI, is scarcity of data, more specifically the quantity and quality of human annotated labels.

%The main challenge for most explored supervised learning approaches for classification of histopathological WSI, is scarcity of labeled data.
%Human annotation of WSIs are costly and time consuming.
A challenge for the supervised learning approaches applied to histopathological WSI is the scarcity of labeled data.
Furthermore, label information for digital WSI is also limited and does not provide details of the affected region at different magnifications, as in dataset BreakHis~\cite{spanhol2016dataset}.
%In contrast to this, manual visual inspection allows the pathologist to identify interesting regions at low magnification and then look at those region specifically with higher magnification.
%In contrast, manual visual inspection where pathologist follows pyramid approach and observes different details at different magnification to identify cancer.
%For instance, the breast cancer histopathology image dataset BreakHis~\cite{spanhol2016dataset} provides abstract classification labels without region specific details for all four WSI of different magnification factor.
%In such scenarios, representations learned through a supervised learning approach are not efficient due to scarcity of labeled data and limited amount of supervision signals in labels.
Representations learned through supervised learning might suffer as such methods typically require a large amount of labeled data.
This can lead to sub-optimal performance on downstream tasks.


%Purpose - Topic sentence for representation learning w/o labels on smaller data
Exploring efficient representation learning on small-scale histopathological WSI data using objectives that do not require labels is a promising approach as it requires a lower amount of labeled data needed to learn successful downstream models.
%Such methods require no labeled data for learning representations, and those representations, in turn, can be used to lower the amount of labeled data needed to learn successful downstream models.
%However, many such methods use human priors to decide on a reasonable objective, which somewhat diminishes the advantage of not requiring human annotated data.
%However, many such methods use human priors to decide on a reasonable objective that requires human effort.

%Enabling efficient representation learning without labels on small-scale of histopathological WSI data is the need of the hours due to scarcity of data and labels.
%Methods in which learning is not supervised by labels for specific objective, tends to learn the representations at full potential.
%These learnt representations helps to improve downstream task performance and reduces the needs of labeled examples.


%Idea to fulfill the purpose - Topic Sentence around self-supervised learning method, MPCS
This work proposes a novel self-supervised learning (SSL) method based on contrastive joint embedding called Magnification Prior Contrastive Similarity (MPCS), to learn efficient representations without labels.
The proposed method uses a magnification factor (a signal from data) to construct positive pairs for contrastive similarity.
%MPSC uses the parameters of a model pretrained on ImageNet~\cite{deng2009imagenet} along with magnification factors to enables self-supervised learning on small-scale datasets.
MPCS uses magnification factors to enable SSL on the small-scale dataset. This work also hypothesizes that reducing human inducted prior in SSL methods enhances representation learning. 
%Some initial investigation of this hypothesis is performed by designing various pair sampling methods e.g. fixed pair, ordered pair, and random pair, ranging from less to more human priors, associated with different inducted human prior to self-supervised pre-training.
%This hypothesis is investigated by designing various pair sampling methods associated with different inducted human prior to self-supervised pre-training.


The proposed method MPCS conducts self-supervised pre-training on histopathological WSI on the BreakHis~\cite{spanhol2016dataset} dataset with two different backbone encoders Efficient-net~\cite{tan2019efficientnet} and dilated ResNet-50~\cite{yu2017dilated}, pre-trained on ImageNet~\cite{deng2009imagenet}.
The effectiveness of the learned representations is assessed by fine-tuning for the downstream task of malignancy classification on multiple public datasets e.g. BACH~\cite{aresta2019bach}, Breast Cancer Cell Dataset~\cite{gelasca2008evaluation} including BreakHis dataset.
%This evaluation is performed by checking how well a model pre-trained with MPCS perform on the downstream task of malignancy classification after fine-tuning using the labeled data at different ratios.
%Further, learned representations are exploited to accomplish the tasks of malignancy classification at different ratio of labeled examples.
The complete approach is depicted in Figure~\ref{fig:mpcs_intro}.
Following are the main contributions: 
\begin{enumerate}
\item Enables self-supervised learning on small-scale histopathology dataset by exploiting a data prior
%\item Demonstrates a label efficient self-supervised learning method and obtains state-of-the-art performance using only 20\% of labeled data.
%\item Outperforming malignancy classification performance over previous works by 3.51\% when using 80\% of the labeled data.
\item Hypothesizes a relation between human inducted prior and data prior for self-supervised representation learning
%\item Presents initial empirical support for the hypothesis by showing that reducing human prior leads to efficient representation learning, which suggests promising further research.
%Empirically supports that reducing human prior leads to efficient representation learning and requires more investigations
%\item Empirical evidence on cross-magnification evaluation to demonstrate magnification invariant representation learning.
\end{enumerate}
With contributions mentioned above, this work demonstrates significantly improved performance on downstream tasks on three public datasets. It provides preliminary empirical support that 1) reducing human-prior leads to efficient representation learning and 2) learning being magnification invariant by cross-magnification evaluation.

==> WACV 2021-MPCS_Arxiv/sections/2_related_work.tex <==
Most efforts in machine learning for histopathological analysis have been using supervised learning.
However, current supervised learning methods struggle when labeled data is scarce~\cite{komura2018machine}.
%However, the field of histopathological classification suffers from scarce amounts of labeled data, which is often a significant problem for purely supervised learning approaches.
Other methods, e.g. pseudo-label and transfer learning, are often used with supervised learning to make up for the lack of labeled data.
%These methods often fall under one or both categories; (i) using unlabeled information or pseudo-labels or (ii) using transfer learning from models trained on other tasks.
Examples of such methods are augmentation~\cite{lin2018scannet} for the first category and feature-extraction and selection~\cite{spanhol2017deep, wang2020breast} for the second.


One public histopathological image dataset that poses such a challenge of data- and label scarcity is BreakHis~\cite{spanhol2016dataset}.
%The dataset consists of magnification based histopathological images on breast cancer BreakHis~\cite{spanhol2016dataset} was released.
%The dataset consists of 2,480 benign and 5,429 malignant images from 82 patients at four different magnification levels (40×, 100×, 200×, 400×).
%The original work suggests two evaluation metrics, image-level accuracy and patient-level accuracy (recognition rate), and presented baseline results.
%Additionally, the original work presents baseline results for the evaluation metrics utilizing a few different strategies.
%These strategies include hand-crafted textural descriptors Local Binary Patterns (LBP)~\cite{ojala2002multiresolution}, Completed Local Binary Patterns (CLBP)~\cite{guo2010completed}, Local Phase Quantization (LPQ)~\cite{ojansivu2008blur}, Grey-Level Co-occurrence Matrix (GLCM)~\cite{haralick1973textural}, Threshold Adjacency Statistics (PFTAS)~\cite{hamilton2007fast}, and Oriented FAST and Rotated Brief (ORB)~\cite{rublee2011orb} with some common machine learning methods (1-NN, QDA, SVM, and Random Forest).
%Following the release of the original dataset, the authors released a work where they tested the effectiveness of using a \ac{CNN} on the dataset~\cite{spanhol2016breast}, though without making use of either of the two methods of handling data scarcity mentioned above.
Many different methods have been applied to the BreakHis~\cite{spanhol2016dataset} dataset, most of which utilize a \ac{CNN} in conjunction with one or both of the methods for handling data scarcity above.

%Recent methods on BreakHis that commonly use \ac{CNN} architectures in fully supervised setting, specifically focusing on transfer learning and customized network architectures employed with specific methods to overcome the data scarcity and other challenges of BreakHis.
%One such method~\cite{spanhol2017deep}, utilizes state-of-the-art \ac{CNN} architectures and uses Deep Convolutional Activation Feature (DeCAF)~\cite{donahue2014decaf} from a CaffeNet~\cite{jia2014caffe} model pretrained on ImageNet.
%DeCAF~\cite{donahue2014decaf} based approaches are resource efficient comparing to training \ac{CNN} from scratch yet performs better than traditional hand-crafted textural descriptors.
%Recent methods on BreakHis that majorly uses customized Convolution Neural Networks (CNN) architectures in fully supervised setting however other works focuses to exploits multiple instance learning considering WSI images and utilizing transfer learning with the state-of-the-art CNNs, respectively.
%Recent methods on BreakHis that majorly uses Convolution Neural Networks (CNN) architectures in fully supervised setting, specifically focusing on transfer learning and customized network architectures employed with specific methods.
%However, other works focuses on exploiting multiple instance learning considering WSI images.
%Recent work focusing transfer learning to overcome the data scarcity challenge of BreakHis~\cite{spanhol2016dataset}, %Deep~\cite{spanhol2017deep} utilizes the state-of-the-art CNN architectures and uses Deep Convolutional Activation Feature for Generic Visual Recognition (DeCAF)~\cite{donahue2014decaf} feature from imageNet pre-trained CaffeNet model is used as only feature extractor to extract features on top of which the parameters of a new classifier learns only for the new classification task.
%The CaffeNet model is used as only feature extractor to extract features on top of which the parameters of a new classifier learns only for the new classification task.

%% Present non-SSL models
%Most approaches to tackle the BreakHis dataset either use transfer learning from models trained on other supervised tasks, train in a supervised learning setting on BreakHis data extended with augmentations, or both.
Table~\ref{tab:previous_work} contains a summary of a few such approaches along with some of the strategies used on BreakHis~\cite{spanhol2016dataset}.
%The table focuses on what models are used, what augmentations are used, if extra training other than fully supervised, if any ensemble or other multiple predictor models are used, and the evaluation protocol.
In the table, custom means a specialized or novel method introduced. Simple augmentations refer to one or more operations among rotation, flipping, cropping, shifting, and zooming.
Another breast cancer dataset is BACH~\cite{aresta2019bach}, on which previous works in transfer learning TL~\cite{vesal2018classification}, patch-based PT~\cite{roy2019patch}, and hybrid networks HN~\cite{yan2020breast} shows performance improvements. Further, the small-scale dataset Breast Cancer Cell Dataset~\cite{gelasca2008evaluation} is also being evaluated for binary tasks in various previous works based on shearlet transform ST~\cite{rezaeilouyeh2016microscopic} and attention methods are ATN~\cite{ilse2018attention} and MATN~\cite{konstantinov2022multi}.

%Such methods include MI~\cite{bayramoglu2016deep}, GLPB~\cite{ataky2020data},  MIL~\cite{sudharshan2019multiple}, A-MIL~\cite{patil2019breast}, and Modified-ResNet~\cite{gupta2021breast}.
%MI~\cite{bayramoglu2016deep} presents a custom multi-task \ac{CNN} that predicts image magnification level in addition to the evaluation metrics which outperforms a magnification specific model.
%GLPB~\cite{ataky2020data} proposes a data augmentation method alongside a custom \ac{CNN} architecture which achieves competent performance.
%MIL~\cite{sudharshan2019multiple} presents a weakly supervised learning framework and investigates the relevance of multiple instance learning.
%A-MIL~\cite{patil2019breast} proposes to use multiple instance learning to train a classifier that provides localization for the potentially interesting regions of the images.
%Modified-ResNet~\cite{gupta2021breast} uses a specialized version of ResNet~\cite{he2016deep} together with  data augmentation to achieve state-of-the-art performance, however the experimental protocol does not explicitly explain any repeating hold-out or cross validation evaluation procedure.

\begin{table}[t]
\caption{Methodologies Used on the BreakHis Dataset.}
\vspace{-0.3cm}
\label{tab:previous_work}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccccc}
\hline
    Work &  Model & Augmented & Extra Training &   Ensemble &  Evaluation\\
\hline
    Deep~\cite{spanhol2016breast} & AlexNet~\cite{krizhevsky2012imagenet} variant & No & No & No & 5 trials\\
    MI~\cite{bayramoglu2016deep} & Custom CNN & Simple & Custom & No & 5-fold\\
    GLPB~\cite{ataky2020data} & TCNN~\cite{andrearczyk2016using} & Custom & No & No & 5-fold\\
    MIL~\cite{sudharshan2019multiple} & Various & MIL~\cite{keeler1991integrated} & No & No & 5 trials\\
    A-MIL~\cite{patil2019breast} & Custom CNN & Simple & No & No & Unclear\\
    MRN~\cite{gupta2021breast} & ResNet~\cite{he2016deep} variant & Simple & No & No & Unclear\\
    MV~\cite{gupta2017breast} & Various & No & No & Voting & 5 trials\\
    SM~\cite{gupta2018sequential} & DenseNet~\cite{huang2017densely} & Simple & Pretrained & XGBoost~\cite{chen2015xgboost} & 3 trials\\
    PI~\cite{gupta2019partially} & ResNet~\cite{he2016deep} & Simple & Pretrained & Custom & 3 trials\\
    TL~\cite{deniz2018transfer} & AlexNet~\cite{krizhevsky2012imagenet} \& VGG16~\cite{simonyan2015very} & No & Pretrained & Two networks & 5-fold\\
    RPDB~\cite{man2020classification} & DenseNet~\cite{huang2017densely} & Simple & AnoGAN~\cite{schlegl2017unsupervised} & No & 5-fold CV\\
    MIM~\cite{benhammou2020breakhis} & Various & Simple & Pretrained & No & Unclear\\
    \textbf{MPCS} & Efficient-net b2~\cite{tan2019efficientnet} & Simple & Custom & No & 5-fold stratified CV\\
\hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}


%Other methods using custom \ac{CNN} architectures to tackle the BreakHis dataset are SW~\cite{spanhol2016breast}, MI~\cite{bayramoglu2016deep}, GLPB~\cite{ataky2020data}, Modified-ResNet~\cite{gupta2021breast}, and SMSE~\cite{sun2021magnificationindependent}.
%SW~\cite{spanhol2016breast} utilizes a AlexNet~\cite{krizhevsky2012imagenet} based architecture with sliding window input format and improves classification performance from previous methods without using hand crafted textural features.
%MI~\cite{bayramoglu2016deep} presents two different custom CNN architectures; a single task CNN to discriminate benign and malignant and a multi-task CNN that additionally predicts image magnification level, results claim that the magnification independent CNN improved the performance of magnification specific model.
%MI~\cite{bayramoglu2016deep} presents a custom multi-task \ac{CNN} that predicts image magnification level in addition to the evaluation metrics which outperforms a magnification specific model.
%GLPB~\cite{ataky2020data} proposes a data augmentation method called Gaussian-Laplacian Pyramid Blending~(GLPB) alongside a custom \ac{CNN} architecture which achieves competent performance.
%Another work using a magnification independent approach, SMSE~\cite{sun2021magnificationindependent} proposes a  similarity-based multi-scale embeddings~(SMSE) framework to train custom \ac{CNN}.
%Particularly, pair loss and triplet loss~\cite{chechik2010large} are leveraged to learn similarity-based embeddings from image pairs or image triplets, which achieves improved recognition rate. In~\cite{gupta2021breast}, modified versions of ResNet~\cite{he2016deep} are used together with data augmentation to claim state-of-the-art performance however experimental protocol does not explicit explains any repeating hold-out or cross validation evaluation procedure.


%Recent Methods focusing multiple instance learning on BreakHis WSI images are A-MIL~\cite{patil2019breast} and MIL~\cite{sudharshan2019multiple}.
%A-MIL~\cite{patil2019breast} proposes to use multiple instance learning to train a classifier that provides %localization for the potentially interesting regions of the images.
%The work, evaluated on single data fold, also makes use of data augmentation to extend the amount of labeled data that is available.
%Another work, MIL~\cite{sudharshan2019multiple} presents a weakly supervised learning framework and investigates the relevance of Multiple Instance Learning~(MIL).
%More specifically, it benchmarks the state-of-the-art MIL methods including MILCNN~\cite{sun2016multiple} and non-parametric methods and shows comparable results to single instance based methods, without need of labeling all the image.





%Other works on BreakHis are based on fusion of multiple methods/models, multiple architectures, and ensemble approaches.
%MV~\cite{gupta2017breast} exploits textural descriptors with ensembles of machine learning method using majority voting.
%Other methods including Partially Independent~\cite{gupta2019partially},  Sequential Modeling~\cite{gupta2018sequential} and~\cite{deniz2018transfer} investigates fusions of CNN with other machine learning methods (SVM, Random Forest) and obtains improved results.
%Another work using two network architectures, DenseNet121-AnoGAN~\cite{man2020classification} uses generative adversarial networks to screen mislabeled patches and DenseNet \ac{CNN} for learning classification however also investigate single model approach using Random Patches with Data Balance (RPDB) inputs.
%Another study,~\cite{benhammou2020breakhis} presents taxonomies of task on BreakHis, specifically focusing magnification independent multi-class classification and complies additional results on fusion approaches and added data processing enabled methods on different folds. 
%Currently lacking a systemic study, transfer learning methods needs to explore in connection with other learning paradigm to counter data scarcity challenges in medical and histopahtological image domain. Employing it or higher performance generalization on BreakHis~\cite{spanhol2016dataset} is one focus of current work.
%The critical fact about experimentation strategy of dataset division followed in mostly all the work Baseline\cite{ojala2002multiresolution} - \cite{rublee2011orb}, MV\cite{gupta2017breast}, SW\cite{spanhol2016breast}, MI\cite{bayramoglu2016deep}, GLPB\cite{ataky2020data}, SMSE\cite{sun2021magnificationindependent}, Deep\cite{spanhol2017deep}, MIL\cite{sudharshan2019multiple}, and Sequential Modeling \cite{gupta2018sequential} on BreakHis dataset\cite{spanhol2016dataset} is splitting the dataset into the train and test set in ratio of 70:30 and repeating the experiments 5-times to take average value. Further, work in~\cite{gupta2021breast} and A-MIL~\cite{patil2019breast} does not indicate repeating folds.
%A careful analysis showcases the weakness of these data splits is mentioned in the Data and Experimental Setup section which also proposes more robust experimentation strategy of dataset division. 

%Several of the works presented in Table \ref{tab:previous_work} use a random 70:30 split of training and test data with repeated trials (\cite{spanhol2016breast, sudharshan2019multiple, gupta2017breast, gupta2018sequential, gupta2019partially}).
%A few other works are ambiguous as to whether full k-fold cross-validation is used or random trials (\cite{patil2019breast, gupta2021breast, benhammou2020breakhis}).
%A careful analysis mentioned in the Data and Experimental Setup section of this work discuss the weakness of random trials and proposes a more robust evaluation strategy.


%A paragraph on recent supervised learning methods for histopathology classification
%Recent methods that mainly uses supervised learning along with some methods to alleviate label scarcity include~\cite{patil2019breast} and~\cite{gupta2021breast}.



% Gustav- Below statement covered above with few details.
%In~\cite{gupta2021breast}, modified versions of ResNet~\cite{he2016deep} are used together with data augmentation to achieve state-of-the-art accuracy on the BreakHis dataset~\cite{spanhol2016dataset}.

%Within deep learning many different approaches have been used in order to train models for classifying tissue using histopathological images.
%Such approaches include feature- extraction and selection~\cite{spanhol2017deep, wang2020breast},  \todo{list approaches like supervised learning and cite them}.

%A paragraph on supervised to SSL
%Now focusing on learning paradigm beyond the fully supervised scenarios where managing data labels are subject to human expertise and effort intensive.
%Even though many methods exist to reduce the amount of labels one need, including data augmentation, these methods often require a human decided prior to work.
%For example, data augmentation needs a human to decide what type of augmentations are beneficial for the given task.
%One method that has been used in many different settings which has been able to reduced both the amount of labeled data and human priors needed is self-supervised learning.
%In the field of feature learning, self-supervised learning refer to methods that make use pseudo-labels to learn features of the data that is hopefully useful for downstream tasks.
%These pseudo-labels can be retrieved from the structure of the data, by obscuring parts of the data to use as labels, by clustering or otherwise grouping data into pseudo-classes, and through many other means.
%The result of self-supervised learning is then often applied to a task in a supervised setting similar to using pre-trained models for transfer learning.  
Another learning paradigm to effectively counter earlier stated data scarcity challenges is self-supervised learning. %It refers to methods that use pseudo-labels retrieved from structural properties of data itself to learn representations.
%Representation learning through self-supervised methods focused on unlabeled data can dramatically reduce the need for annotations by human experts.
%A common approach to self-supervised learning is to optimize the similarity of some extracted features.
Representation learning from self-supervised learning paradigms for computer vision can be categorized majorly as (i) Joint Embedding Architecture \& Method (JEAM) (\cite{chen2020simple, grill2020bootstrap, caron2020unsupervised, zbontar2021barlow}), (ii) Prediction Methods (\cite{veeling2018rotation, noroozi2016unsupervised, doersch2015unsupervised}), and loosely (iii) Reconstruction Methods~(\cite{kingma2013auto, goodfellow2014generative}).
%JEAM is primarily conceptualized over multiple views of input images, exploitation of embedding capabilities of joint architectures, and specialized loss objectives have shown recent advances in self-supervision.
Specifically, JEAM can be divided further with each subdivision providing many interesting works; (i)~Contrastive Methods (PIRL~\cite{misra2020self}, SimCLR~\cite{chen2020simple}, SimCLRv2~\cite{chen2020big}, MoCo~\cite{he2020momentum}), (ii)~Distillation (BYOL~\cite{grill2020bootstrap}, SimSiam~\cite{chen2021exploring}), (iii)~Quantization (SwAV~\cite{caron2020unsupervised}, DeepCluster~\cite{caron2018deep}), and (iv)~Information Maximization (Barlow Twins~\cite{zbontar2021barlow}, VICReg~\cite{bardes2021vicreg}).
Of these divisions, this work focuses on contrastive methods.
%The works SimCLR~\cite{chen2020simple}, SimCLRv2~\cite{chen2020big}, and MoCo~\cite{he2020momentum} formalizes contrastive JEAM by providing frameworks for learning similarity between positive pair of distorted/transformed views from same images and dissimilarity from negative pairs from different images.
%The methods vary by how they manage the large pool of negative pairs, with SimCLR using a larger batch size and MoCo using a momentum encoder.

%The distillation method BYOL~\cite{grill2020bootstrap} based on knowledge distillation~\cite{hinton2015distilling} of moving averaged parameter sharing from source trainable network to target network and SimSiam~\cite{chen2021exploring} are based self-distillation added MLP enabled Siamese network~\cite{bromley1993signature} uses stop-grad to prevent collapses.

%Quantization JEAM SwAV~\cite{caron2020unsupervised} employs cluster assignments on representation vectors \& DeepCluster~\cite{caron2018deep} performs cluster assignments as pseudo-labels for learning.

%Information Maximization JEAM Barlow Twins~\cite{zbontar2021barlow} prevents informational collapse by utilizing the cross-correlation matrix to make embedding vectors similar while minimizing the redundancy between it and VICReg~\cite{bardes2021vicreg} additionally focuses on regularization through variance of both embeddings separately across each dimension and de-correlations over each pair of variables.


%The medical image domain has also shown advances in self-supervised learning to counter the challenge of mitigating label scarcity in general.
%The self-supervised methods are MRI~\cite{bai2019self}, Rubik Cube~\cite{zhuang2019self} and Rubik Cube$+$~\cite{zhu2020rubik} on 3D medical images, \cite{spitzer2018improving} on human brains.

Recently, contrastive JEAM has been tailored for medical images. Contrastive learning on digital pathology DPCL~\cite{ciga2022self} applies contrastive learning and shows improvement in the breast cancer dataset~\cite{aresta2019bach}. 
In~MICLe~\cite{azizi2021big}, which is based on SimCLR~\cite{chen2020simple}, multiple instance contrastive learning is applied by enabling input views from several image instances of the same patient.
Another work from contrastive methods on histopathology is DRL~\cite{xu2020dataefficient}.
%which learns representations based on local structure heterogeneity and global context homogeneity over noise contrastive estimation.
%It obtains state-of-the-art performance on the GlaS~\cite{sirinukunwattana2017gland} and PCam~\cite{veeling2018rotation} datasets. An
Other applications making use of contrastive JEAM are chest X-rays~\cite{sowrirajan2021moco, liu2019align}, CT scans for COVID-19~\cite{he2020sample}, 3d-Radiomic~\cite{li2021imbalance}, and Radiograph~\cite{zhou2020comparing}.
A work using contrastive JEAM on the BreakHis dataset is SMSE~\cite{sun2021magnificationindependent}, which trains the network using pair and triplet losses.
%It is clear that contrastive JEAM for feature learning has progressed in histopathology images.
%Currently, contrastive learning suffers from requiring a large amount of data for pre-training and specialized human knowledge to provide prior and annotations.
SSL methods including JEAM require large-size data. Thus applying the contrastive JEAM paradigm on small datasets with the reduced human dependency of prior is an open challenge and interest of this work.




%\todo - First non-CL SSL which are in medical but not histopathological, then CL based SSL but not hisporathlogical it will inlcude azizi also, then CL on histopathological images but not BreakHis, then CL on BreakHis, then reason for ourt method.





%There are many vastly different methods that build on the idea to optimize similarity of learned features.
%Such methods include pair-loss~, triplet-loss~\cite{chechik2010large}, contrastive learning, knowledge distillation~\cite{hinton2015distilling}, Siamese networks~\cite{bromley1993signature}, and many others.


%Recent works following contrastive joint embedding methods successfully include SimCLR~\cite{chen2020simple}, SimCLRv2 distillation~\cite{chen2020big},  BYOL~\cite{grill2020bootstrap}, MoCo~\cite{he2020momentum}, and SimSiam~\cite{chen2021exploring}.
%SimCLR presents a simplified framework for contrastive learning in the computer vision domain.
%SimCLRv2 distillation uses an updated version of the SimCLR framework to train a larger model that is then fine-tuned and used for knowledge distillation of a smaller model.
%BYOL presents a new method of self-supervision similar to knowledge distillation where one network is trained to predict the features of another networks whose parameters are defined by a moving average of the trained network.
%MoCo presents a \todo.
%SimSiam presents a version of Siamese networks trained such that an MLP should predict the output of an encoder given an augmented image given the output of the same encoder given another augmentation of the same image; the training of this is prevented from collapsing by a stop-grad operation.


%Contrastive learning extension for medical images are explored on chest X-ray~\cite{sowrirajan2021moco`} and \cite{liu2019align}, CT scans for COVID-19 \cite{he2020sample}, 3d radiomic \cite{li2021imbalance}, and radiograph \cite{zhou2020comparing}.




%One method for self-supervised learning that has been used more, both within deep learning in general and histopathology classification specifically, is contrastive learning.
%In general contrastive learning is used to learn intermediate features that can then be used by a downstream prediction model.
%This is done by minimizing the feature space distance between samples from the same group and maximizing the distance between samples of different groups.
%An important step of training with contrastive learning is to decide how the input samples are grouped.
%This can be done in a completely supervised fashion, using human labeled data~\tocite{} or, more commonly, in a self-supervised setting, where the groups are not determined by labels.
%The most common self-supervised version of contrastive learning is where data points are grouped with augmented versions of that same data point\tocite{}.
%However, other methods exists that often makes use of unlabeled information,\todo{more grouping methods}.

%A paragraph on recent self-supervised methods for histopathology classification
%Self-supervised learning has recently been successfully applied to histopathology classification, often together with some of the previously mentioned techniques for mitigating label scarcity.
%Recent methods that have used self-supervised learning include~\cite{xu2020dataefficient}, \cite{sun2021magnificationindependent}, and~\cite{azizi2021big}.


%In~\cite{xu2020dataefficient}, data augmentation by image deformation is used to create groups for use with contrastive learning, and achieves results comparable to state-of-the-art in low data settings on the GlaS PCam dataset~\cite{veeling2018rotation}.


%In~\cite{sun2021magnificationindependent}, the groups for contrastive learning are collected by grouping images at different magnification levels for the same samples in combination with data augmentation, which has the additional benefit of providing some level of magnification independence to prediction.
%In both works contrastive learning is used to pretrain a feature extraction model which is then used to train downstream models in a supervised setting.

, 

==> WACV 2021-MPCS_Arxiv/sections/3_methodology.tex <==
%This work primarily aims for novel self-supervised pre-training method development to perform malignancy classification on whole-slide histopathological images (WSI) in a limited labeled data scenario.
The primary focus of this work is to introduce a novel self-supervised pre-training method with the aim is to learn representations from data without labels, while using supervision signals from data, e.g., magnification factor and using inductive transfer from ImageNet~\cite{deng2009imagenet} pre-trained weights.
%to enhance the accuracy of malignancy classification on Whole-slide Histopathological Images (WSI) with limited labels.
%The aim is to learn representations from data without labels and use supervision signals from data, e.g., magnification factor.
%To help overcome the unlabeled data scarcity, the work aims to effectively utilize inductive transfer from the domain of ImageNet~\cite{deng2009imagenet}.
% More specifically, this work focuses on following two objectives:
% \begin{enumerate}
%     \item Exploiting inductive transfer learning from ImageNet\cite{deng2009imagenet} pre-trained Efficient-net \cite{tan2019efficientnet} for .
%     \item Developing a self-supervision paradigm based novel pretraining method for learning visual representations without explicit human supervised labels for achieving robust performance on downstream task with minimal (only 20\%) labeled data.
% \end{enumerate}



%Contribution
% - Robust improved SOTA on supervised setting
% - Enabling SSL on small scale dataset by exploiting prior from data allowing to obtain downstream task performance better than previous arts
% - SSL story on non-natural images where human prior in terms of  augmentation doesn't apply - overcoming of general SSL weakness
% - Benchmarking SSL on Efficient-net architecture

% future - Exploring unsupervised TL and SSL TL where unsupervised inductive in the case.
 
\subsection{Inductive Transfer Learning}

% Neural networks are proven universal function approximators~\cite{scarselli1998universal} with sufficient parameters.
% However they suffer from poor performance generalization on unseen data from either from same distribution or out of distribution.
% when training data is in scarcity. 


% This is a long-standing challenge in the field.
% However, transfer learning methods~\cite{yosinski2014transferable} reduces this barrier by allowing a model to use the knowledge learned on source domain to apply on target domain. 
% In general, transfer learning is effective to obtain performance improvement through learned representations but optimal outcome is subject to correct choice of method, network architecture, and characteristics of source domain. 
% Recently, transfer learning based methods~\cite{spanhol2017deep} and~\cite{patil2019breast} have been employed on the BreakHis dataset~\cite{spanhol2016dataset}, however it has not been explored comprehensively. 

% Current work reformulates the challenge of obtaining higher performance generalization on unseen data from either from same distribution or out of distribution using transfer learning~\cite{zhuang2020comprehensive}.
% % Given the fact that BreakHis~\cite{spanhol2016dataset} is small scale and class imbalanced dataset. 
% Often training large-scale CNNs from scratch suffers overfitting. On the other hand, simpler networks fail to learn due to underfitting. 
% Furthermore, the non-availability of the same domain large-scale dataset with labels end the possibility of homogeneous transfer learning. 
Given the fact that BreakHis~\cite{spanhol2016dataset} is a small-scale and class-imbalanced dataset, this work hypothesizes a constraint case of inductive transfer for representation learning by initializing encoder ImageNet~\cite{deng2009imagenet} pre-trained weights.
%Further learned representations, to utilize in finetune on same and other breast cancer datasets. 
% To define transfer learning in context of neural networks based models concretely \cite{zhuang2020comprehensive}, A domain $\displaystyle \mathcal{D}$ $=\{\displaystyle \mathcal{X},$ $\displaystyle \mathcal{P}(X) \}$ with input feature-space $\displaystyle \mathcal{X}$ and a marginal probability distribution $\displaystyle \mathcal{P}(X)$: $X=\{x_1,..,x_n\}$ \in \hspace{0.5em} $\displaystyle \mathcal{X}$ where n is size of example set, and a task $\displaystyle \mathcal{T=\{Y,}$ $f_\theta(x)\}$ where $\displaystyle \mathcal{Y}$ is output label space and $f_\theta: \displaystyle \mathcal{X} \to \displaystyle \mathcal{Y}$, an objective predictive function serves prediction of corresponding label $f_\theta(x)$ of instance of $x$ and $\displaystyle \mathcal{\theta}$ is learning parameter(s) associated with architecture of learning device, e.g. neural networks, learns through optimization over predictive function. In supervised learning, $\displaystyle \theta_{MLE}$, notifies maximization the likelihood estimate for the parameters $\displaystyle \mathcal{\theta}$ which corresponds with finding the parameters $\displaystyle \mathcal{\theta}$ for which the likelihood of the input feature-space $\displaystyle \mathcal{X}$ is maximised during training. The learnable task $\displaystyle \mathcal{T}$ is trained on data pairs $\{x_i,y_i\}$ where $x_i \in X $ and $y_i \in \displaystyle \mathcal{Y}$.
% Thus, considering likelihood estimate for the parameters and predictive function as conditional probability estimator are defined approximately as: $$ \displaystyle \theta_{MLE} = \arg \max_{\theta} \log \prod_{i=1}^{N} p(y_i|x_i,\theta)$$ $$ \displaystyle f_\theta(x) = p(y_i|x_i,\theta)$$ where $p(y_i|x_i,\theta)$ is conditional probability to predict label $y_i$ for given input $x_i$ and parameter $\displaystyle \mathcal{\theta}$.\\
%The objective predictive function $f_\theta: \displaystyle \mathcal{X} \to \displaystyle \mathcal{Y}$ aims to learn
%In this work, a heterogeneous source domain dataset \ie ImageNet~\cite{deng2009imagenet} is used to train a multi-class large-scale network that disseminates common yet robust knowledge about visual representation to small-scale target domain dataset \ie BreakHis\cite{spanhol2016dataset} for self-supervised representation learning and downstream tasks. Specifically, Efficient-net~\cite{tan2019efficientnet} b2 and ResNet-50~\cite{yu2017dilated} encoders are used.
% To define transfer learning~\cite{zhuang2020comprehensive} in the context of this work, the source and target domains and tasks are defined as following,
% Consider the source domain $\displaystyle {\mathcal {D}}^{S}$ $=\{\displaystyle \mathcal{X^S},$ $\displaystyle \mathcal{P^S}(X^S) \}$ associated with ImageNet\cite{deng2009imagenet}, with input feature-space $\displaystyle \mathcal{X^S}$ and a marginal probability distribution $\displaystyle \mathcal{P^S}(X^S)$.
% %: X^S=\{x^S_1,..,x^S_{n_S}\}$ $\in$ \hspace{0.1 cm} $\displaystyle \mathcal{X^S}$ where $n_S$ is size of example set which is large indeed, and 
% The source task $\displaystyle \mathcal{T^S=\{Y^S,} f^S_\theta(x^S)\}$ is classification of $1000$ categories of visual objects where $\displaystyle \mathcal{Y^S}$ is output label space and $f^S_\theta: \displaystyle \mathcal{X^S} \to \displaystyle \mathcal{Y^S}$, an objective predictive function and $\displaystyle \mathcal{\theta}$ represents the parameters.
% To accomplish the task, the objective function learns the patterns in the data by modifying the parameters until the optimal values of the parameters are achieved \ie $\theta^{S}^{*}$.
% %associated with architecture of chosen \ac{CNN} Efficient-net \cite{tan2019efficientnet}, learns through task $\displaystyle \mathcal{T^S}$ optimization over predictive function $f^S_\theta$
% % Similarly, the target domain $\displaystyle {\mathcal {D}}^{T}$ $=\{\displaystyle \mathcal{X^T},$ $\displaystyle \mathcal{P^T}(X^T) \}$ is BreakHis\cite{spanhol2016dataset} with input feature-space $\displaystyle \mathcal{X^T}$ and a marginal probability distribution $\displaystyle \mathcal{P^T}(X^T)$: $X^T=\{x^T_1,..,x^T_{n_T}\}$ $\in$ \hspace{0.1 cm} $\displaystyle \mathcal{X^T}$ where $n_T$ is size of example set which is smaller than source domain, and a task $\displaystyle \mathcal{T^T=\{Y^T,} f^T_\theta(x^T)\}$ is classification of malignant and benign categories of tumor where $\displaystyle \mathcal{Y^T}$ is output label space and $f^T_\theta: \displaystyle \mathcal{X^T} \to \displaystyle \mathcal{Y^T}$, an objective predictive function and $\displaystyle \mathcal{\theta}$ is learning parameter(s) associated with architecture of chosen CNN same as in source domain, learns through task $\displaystyle \mathcal{T^T}$ optimization over predictive function $f^T_\theta$
% Similarly the target domain $\displaystyle {\mathcal {D}}^{T}$ is associated with the BreakHis\cite{spanhol2016dataset} dataset which is smaller than the source data, and the target task $\displaystyle \mathcal{T^T}$ is to classify malignant and benign categories of tumor. 
% In order to accomplish the target task, there are two possible conditions,
% \begin{itemize}
%     \item Condition 1: $\displaystyle \mathcal{T^S} \perp\!\!\!\perp \displaystyle \mathcal{T^T}$, \ie Independent Tasks $$\displaystyle {\theta^S \to \theta^{S*}} , \hspace{0.3cm}{\theta^T \to \theta^{T*}}$$  
%     Given, size of source data ($n_S$) $>>$ size of target data ($n_T$), 
%     %$n_S$ being absolute large and $n_T$ being absolute small, for same $|\displaystyle {\theta}|$,
%     $\displaystyle {\theta^{S*}}$ generalizes well but $\displaystyle {\theta^{T*}$ does not due to insufficient representation learning in absence of transfer learning.
%     \item Condition 2: $\displaystyle \mathcal{T^S}$$\tikzmarknode[strike out,draw]{1}{\perp\!\!\!\perp}$$\displaystyle \mathcal{T^T}$ \ie Conditional dependence by Inductive Transfer) $$\displaystyle {\theta^S \to \theta^{S*}} , \hspace{0.3cm} \mathbf{\displaystyle \theta^{S*} \to \theta^{T*}}$$  
%     Given $n_S >> n_T$, 
%     %although $n_T$ being smaller, for same $|\displaystyle {\theta}|$, 
%     $\displaystyle {\theta^{S*}}$ generalizes well and initialization  of $\displaystyle {\theta^T}$ by $\displaystyle {\theta^{S*}}$ through inductive transfer disseminate knowledge of usable representations thus during task $\displaystyle \mathcal{T^T}$, $\displaystyle {\theta^{T*}}$ obtains performance generalization by preventing overfit condition.
% \end{itemize}
In this work, the inductive transfer (i) helps to obtain improved performance on the downstream task of malignancy classification and (ii) enables self-supervised pre-training using the proposed method on the small-scale dataset.% for the downstream task in a limited labeled data setting.   
%in a fully supervised setting
%\begin{itemize}
%\color{blue}
%\item TODO - write about how transfer learning is used in this work
%    \begin{itemize}
%    \color{blue}
%        \item In terms of Imagenet pretrained models are used 
%        \item 80 percent , 20 percent experiments ??
%    \end{itemize}

%\end{itemize}
    %\item For given $n_S >>>> n_T$ where $n_S$ being very large and considering learnable task $\displaystyle \mathcal{T^S}$ and learnable task $\displaystyle \mathcal{T^T}$ independent optimizes; $$\displaystyle {\theta^S \to \theta^S_{MLE}}$$

  
    %\item The target domain $\displaystyle {\mathcal {D}}_{T}$ is BreakHis WSI \cite{spanhol2016dataset}, learning task  $\displaystyle {\mathcal {T}}_{T}$ is binary classification to identify the carcinoma,  and corresponding predictive function is $f_{T_\theta}: \displaystyle \mathcal{X_T} \to \displaystyle \mathcal{Y_T}$
    %The employed transfer learning method considered as
    %\item A constrained case of inductive transfer is hypothesized where input feature-space $ \displaystyle \mathcal{X_S}$ of source domain $\displaystyle {\mathcal {D}}_{S}$ and input feature-space $ \displaystyle \mathcal{X_T}$ of target domain $\displaystyle {\mathcal {D}}_{T}$ are distinct ($ \displaystyle \mathcal{X_S}$ $\neq$ $ \displaystyle \mathcal{X_T}$) and also same applies to output label spaces ($ \displaystyle \mathcal{Y_S}$ $\neq$ $ \displaystyle \mathcal{Y_T}$)
    %\item Parameter $\displaystyle \mathcal{\theta}$ in the current work setting corresponds to the learning parameters of architecture of Efficient-net \cite{tan2019efficientnet}.
    %\item For given size of trainsets for domains $\displaystyle {\mathcal {D}}_{S}$ and $\displaystyle {\mathcal {D}}_{T}$ where $n_1 >>>> n_2$, thus predictive function $f_{S_\theta}$ learns representation during task $\displaystyle {\mathcal {T}}_{S}$ on domain $\displaystyle {\mathcal {D}}_{S}$ and disseminate knowledge through learned parameter $\displaystyle \mathcal{\theta}$. This knowledge predictive function $f_{T_\theta}$ apply for task $\displaystyle {\mathcal {T}}_{T}$ on domain $\displaystyle {\mathcal {D}}_{T}$ to obtain optimal performance generalization.    




%is also different besides, output domain and knowledge transfer is paramateric in nature.



%Specifically in current context of transfer learning, we employ a constrained case of inductive transfer where input space is also different besides, output domain and knowledge transfer is parametric in nature


%Point 1 - Define concretely the TL ~ Representation learning, target downstream task ,

%Point 2 - Case specific - Imagenet pretrained Efcientet architecture used - describe it
%Point 3 - Further DT case specific - Supervised, SSL based 


%In this work, transfer learning is applied in both supervised as well as self-supervised settings.
%Already trained networks on ImageNet \cite{imagenet_cvpr09}, which is a very large multi-label image database, are utilized here for material type classification.
%These are further discussed in sec. \ref{supervised} and sec. \ref{selfsupervised}.
\subsection{Self-supervised Method - Magnification Prior Contrastive Similarity} \label{ssl}
\begin{comment}
Recent advances in Contrastive Joint Embedding Embedding Architecture \& Method (JEAM) SimCLR~\cite{chen2020simple}-\cite{chen2020big}, and other methods are robust for representation learning and obtaining state-of-the-art performance.
%However, these methods requires large-scale data and extensive human knowledge in terms of strong prior due to the mechanism of learning based on the creation of distorted views of input visual and similarity learning objectives on those views.
%This challenge does exist in other approaches of JEAM also.
%One of the main reasons behind the success of the current state of contrastive JEAM approach on natural visual domain ImageNet~\cite{deng2009imagenet} is human inducted prior.
%Because humans are naturally efficient in knowledge over natural visual concepts significantly contributes to discriminative yet co-related views of visual input through augmentation-based transformation methods.
This work hypothesizes that inducted humans prior suppress the potential of networks to learn in a self-supervised manner more independently towards imitating biological intelligence.
The limitation imposed due to the needs of strong human prior is more recognizable considering beyond the natural visual concept based domains like medical imaging, microscopic images of pathology, and others.
Human knowledge and perception of such domains are relatively limited and fail to compile domain-specific characteristics to create effective transformations for distorted views.
Specifically, BreakHis dataset~\cite{spanhol2016dataset} contains Whole Slide Images (WSI) of four magnifications and affected regions present only on some parts of WSI.
Further, the affected region is not necessarily located in the center of WSI.
Applying transformations from natural visual concept domains to BreakHis does not tend to learn optimal representations because visual and textural properties are very different, including location, size, shape, background-foreground, and concrete definition of objects.
Thus network needs to learn representations by self-attention on affected regions across magnifications that are invariant to location, global context, \& several other geometric characteristics.
So stronger human prior prevents networks from learning and focusing on self-attention.  

Knowing the fact from the literature that human-prior is required for the current state of self-supervised methods, this work focuses on i) exploiting self-supervision signal \& prior from data, i.e., magnification factor to reduce the human prior, and  ii) enabling representation learning on small-scale dataset~\cite{spanhol2016dataset} by utilizing transfer learning and using augmentation based transformation in a specific arrangement.
\end{comment}
Magnification Prior Contrastive Similarity (MPCS) method formulates self-supervised pre-training to learn representations on microscopic Histopathology WSI without labels on small-scale data. The main objective of MPCS is to lower the amount of labeled data needed for the downstream task to address challenges in supervised learning. 

MPCS construct pairs of distinct views considering characteristics of microscopic histopathology WSI (H-WSI) for contrastive similarity-based pre-training.
Microscopic H-WSI structural properties are different from natural visual macroscopic images~\cite{deng2009imagenet} (vehicles, cats, or dogs) in terms of location, size, shape, background-foreground, and concrete definition of objects.
Unlike SimCLR~\cite{chen2020simple} where pairs of distinct views from the input image is constructed by human-centered augmentations, MPCS constructs pair of distinct views using pair sampling methods based on the signal from data itself i.e. magnification factor in BreakHis~\cite{spanhol2016dataset}. 
Two H-WSI from different magnification factors of the same sample makes a pair. 
Utilizing prior from data~(magnification factor) enables meaningful contrastive learning on histopathology H-WSI and reduces dependency over human inducted prior.
Further, tumor-affected regions in H-WSI are characterized by format and highly abnormal amounts of nuclei. 
Such affected regions are promising in all the H-WSIs of different magnification for the same sample.
Thus, affected regions being common and size invariant in positive pair of a sample allow learning contrastive similarity by region attentions.

%MPCS effectiveness on the small-scale dataset is obtained through inductive transfer learning of pre-trained ImageNet~\cite{deng2009imagenet} model and applying a uniform instance of augmentation to both the views of pair during self-supervised pre-training.  

\begin{figure}[t]
    \centering
    \includegraphics[width =0.6\linewidth]{sections/figures/ssl_method_mpcs.png}
    \vspace{-0.2cm}
    \caption{Magnification Prior Contrastive Similarity method explained}
    \label{fig:ssl_mpcs}
    \vspace{-4mm}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.6\linewidth]{sections/figures/human_prior_strategy.png}
    \vspace{-0.2cm}
    \caption{Strategies for pair sampling based on inducted Human Prior(HP). Added measure to prevent mode collapse in pre-training by $1^{st} view \neq 2^{nd} view$ in all strategies.}
    \label{fig:human_prior}
    \vspace{-5mm}
\end{figure}

Current work also hypothesizes that reduced human-prior in the pre-training method provides an enhanced degree of freedom to the method that can increase the potential of the network to learn efficient representations in a self-supervised approach. To investigate, three strategies for pair sampling are formulated based on inducted human prior. The number of human decisions defines the level of inducted human-prior (HP) during pair sampling. As explained in Figure~\ref{fig:human_prior}, in Fixed Pair, decisions to choose magnification factor for both views are by human, thus making strong human-prior. In Ordered Pair, only the second view of the pair is chosen by a human using a look-up table, making weaker human prior. In Random Pair, no human prior inducted and magnification factor for both views are sampled randomly. Further, Figure~\ref{fig:degrre_of_freedom} demonstrates the Degree of Freedom (DoF) for the method where the Fixed Pair strategy provides no DoF, Order Pair provides one DoF, and Random Pair provides 2 DoF to the method. 

%Exploring efficient representation learning on small-scale histopathological WSI data using objectives that does not require labels is therefore a promising approach. Such methods requires no labeled data for learning representations, and those representations in turn can be used to lower the amount of labeled data needed to learn successful downstream models. However, many such methods make use of human priors to decide on a good objective which requires human effort.


%The proposed method, Magnification Prior Contrastive Similarity (MPCS), follows contrastive loss from the Contrastive Joint Embedding Architecture \& method.
%It SimCLR~\cite{chen2020simple} and inducts supervision signal magnification factor, significantly reducing human prior.
%This work formulates three strategies of providing Human Prior (HP) over magnification factor in a proposed method based on Degree of Freedom (DoF) self-supervised method receives.
%It helps to investigate and prove the hypothesis about reduced human-prior to increase the learning potential of the network.
%These variants Fixed Pair, Ordered Pair, and Random Pair are explained in Figure ~\ref{fig:human_prior} and their relation with the degree of freedom of MPCS is explained in Figure~\ref{fig:degrre_of_freedom}.
%With moderate amount of data availability in terms of reflectance and depth images as pair, we proposes a method, Depth Contrast, based on normalized temperature-scaled cross entropy loss from SimCLR \cite{chen2020simple}. It models the two transformed views of input images from a pair of reflectance and depth image respectively and intend to maximizes the agreement between the stated views of same data example through contrastive loss. Derived from SimCLR \cite{chen2020simple}, following are the components for Depth Contrast, mentioned in Figure \ref{fig:depth_contrast_fig}.

In MPCS, to formulate a batch of $2N$ views, randomly sampled batch of $N$ sets of input $X=\{X^{(1)}, X^{(2)}, ..., X^{(N)}\}$ are considered where each set of input $X^{(i)}=\{x^{(i)}_{40}, x^{(i)}_{100}, x^{(i)}_{200}, x^{(i)}_{400}\}$ contains the images corresponding to four magnification factors.
Positive pair of views is constructed based on a selection strategy of pair sampling which contains two views from the same example of different magnification. Further, similarity maximizes (loss minimizes) by an objective defined by the contrastive loss in Eq.~\ref{eq:loss}). MPCS is demonstrated in Figure~\ref{fig:ssl_mpcs} and components are explained below.

\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.8\linewidth]{sections/figures/magnification_prior_contrastive_similarity_degree_of_freedom_v2.png}
    \vspace{-0.2cm}
    \caption{Relation between inducted Human Prior (HP) of magnification and Degree of Freedom (DoF) for method}
    \label{fig:degrre_of_freedom}
    \vspace{-4mm}
\end{figure}
\begin{itemize}
    \item A \textit{domain specific human prior} module $P_h(X \to X_\mathrm{MF})$: $X=\{x_{40}, x_{100}, x_{200}, x_{400}\}$ that exploits supervision signal from data i.e. magnification and samples the two views $X_\mathrm{MF}=$(\textbf{$x_\mathrm{MF1}$}, \textbf{$x_\mathrm{MF2}$}) of different magnifications to construct pair based on employed strategy of pair sampling shown in step 1 of Figure~\ref{fig:ssl_mpcs}. \vspace{-0.2cm}
    \item A \textit{uniform stochastic transformation} based module $\displaystyle \mathcal{T_U}(X_\mathrm{MF} \to \tilde{X}_\mathrm{MF})$ that uniformly transforms both views from $X_\mathrm{MF}=$(\textbf{$x_\mathrm{MF1}$}, \textbf{$x_\mathrm{MF2}$}) to $\tilde{X}_\mathrm{MF}=$ (\textbf{$\tilde{x}_\mathrm{MF1}$}, \textbf{$\tilde{x}_\mathrm{MF2}$}) of positive pair by sampled augmentation transformations scheme shown in step 2 of Figure~\ref{fig:ssl_mpcs}.\vspace{-0.2cm}
    %Current methods applies uniform transformation of sampled augmentation scheme to scale pre-training on small-scale dataset BreakHis~\cite{spanhol2016dataset} whereas SimCLR~\cite{chen2020simple} relies on augmentations to created distinct distorted views of input to construct pair which indicates strong human prior.
    \item  A neural network \textit{base encoder} \textit{f}(·) which yields representations from transformed views of pair. It obtains $h_\mathrm{MF1}$ = \textit{f}($\tilde{x}_\mathrm{MF1}$) = encoder-network($\tilde{x}_\mathrm{MF1}$) and $h_\mathrm{MF2}$ = \textit{f}($\tilde{x}_\mathrm{MF2}$) = encoder-network($\tilde{x}_\mathrm{MF2}$) where $h_\mathrm{MF1}$, $h_\mathrm{MF2} \in \mathbb{R}^d$ are the output after the respective average pooling layers, shown in step 3 of Figure~\ref{fig:ssl_mpcs}.\vspace{-0.2cm}
    \item A small-scale \textit{MLP projection head} \textit{g}(·) that maps representations to the latent space where contrastive loss is applied, shown in step 4 of Figure~\ref{fig:ssl_mpcs}.
    A multi-layer perceptron with single hidden layer to obtain $z_\mathrm{MF1}$ = \textit{g}($h_\mathrm{MF1}$) = $W^{(2)}\sigma(W^{(1)}{h_\mathrm{MF1}})$ and $z_\mathrm{MF2}$ = \textit{g}($h_\mathrm{MF2}$) = $W^{(2)}\sigma(W^{(1)}{h_\mathrm{MF2}})$ where $\sigma$ is ReLU.\vspace{-0.2cm}
    \item A \textit{contrastive loss function}, normalized temperature-scaled cross entropy loss (NT-Xent) from SimCLR is defined for a contrastive prediction, shown in step 5 of Figure~\ref{fig:ssl_mpcs}.
    For given a set \textbf{$\tilde{x}_{k}$} including a positive pair examples \textbf{$\tilde{x}_\mathrm{MF1}$} and \textbf{$\tilde{x}_\mathrm{MF2}$}, the contrastive prediction task tends to find \textbf{$\tilde{x}_\mathrm{MF2}$} in \{${\mathbf{\tilde{x}_{k}}}\}_{k\neq MF1}$ for the given \textbf{$\tilde{x}_\mathrm{MF1}$}.
\end{itemize}

The loss function for a positive pair of examples (MF1, MF2) is defined as
\begin{equation}
    L_\mathrm{MF1,MF2} = -\log \dfrac{\exp(sim(\boldsymbol{z}_\mathrm{MF1},\boldsymbol{z}_\mathrm{MF2})/\tau)} {\sum_{k =1}^{2N} 1_{[k \neq MF1]} exp(sim(\boldsymbol{z}_\mathrm{MF1},\boldsymbol{z}_{k})/\tau)}
    %\vspace{-1em} 
    \label{eq:loss}
\end{equation}
\begin{comment}

\begin{equation}
   sim(\boldsymbol{z}_\mathrm{MF1},\boldsymbol{z}_\mathrm{MF2}) = \dfrac{\boldsymbol{z}^T_\mathrm{MF1}  \boldsymbol{z}_\mathrm{MF2}} {\parallel sim(\boldsymbol{z}_\mathrm{MF1}) \parallel \parallel sim(\boldsymbol{z}_\mathrm{MF2}) \parallel}
   \vspace{-1em}
\end{equation}

\begin{equation}
   sim(\boldsymbol{z}_\mathrm{MF1},\boldsymbol{z}_{k}) = \dfrac{\boldsymbol{z}^T_\mathrm{MF1}  \boldsymbol{z}_{k}} {\parallel sim(\boldsymbol{z}_\mathrm{MF1}) \parallel \parallel sim(\boldsymbol{z}_{k}) \parallel}
\end{equation}
\end{comment}

In Eq.~(\ref{eq:loss}), where $1_{[k \neq MF1]} \in {0, 1}$ is an indicator evaluating to 1 if $k \neq i$.
%Equation 2 and 3 defines dot product between $l_2$ normalized respective quantities and $\tau$ defines the temperature parameter.
%VICReg follows recent trends in self-supervised learning Caron et al. (2020); Grill et al. (2020);
%Chen & He (2020); Zbontar et al. (2021); Chen et al. (2020a) and is based on a joint embedding
%architecture. Contrary to many previous approaches, our architecture may be completely symmetric
%or completely asymmetric with no shared structure or parameters between the two branches.

%To counter the above stated challenges, current work hypothesize that human prior on natural visual concepts, 
%become interinis weakness for self supervierion and it prevent NN to learn representaiuton at full potential. 
%This fact is overlooked for natual vision domain becuase human knowledge and ability to provide prior is high but beyond
%the natual visual concept based domains, where Human based prior is limited by knowlsdge, perception greatly effect the potential of NN to learn repesentations.
%We can more understnd this fact by example of human prior for natual vision and beyong vision (BreakHis)

%Representations from several self-supervised learning paradigm i.e. contrastive method~\cite{chen2020simple} \& \cite{chen2020big}, knowledge distillation~\cite{grill2020bootstrap} \& \cite{chen2021exploring}, and prediction methods~\cite{veeling2018rotation} shown success in reducing human supervision of annotations for downstream tasks. In particular, contrastive reconstructions 

%Self-supervised learning for vision domain are great in sense of reducing human supervision in terms of annotations of images. They are mainly three approaches, i.e. predictive[REFERENCE], contrastive embedding architectures[REFERENCES], and knowledge distillation[REFERENCES]. However, current state of self-supervised has two important components, distorted views inputs and similarity learning objective on those views. Further, one common requirement for current state of self-supervised learning relates to  unlabeled but massive amount of data.\\
%While the reason of effectively creation of distorted views [REFERENCE] are the one of the basis behind the success for self-supervised methods for natural visual concepts[REFERENCES]. Primary reason is Human being naturally efficient in understanding natural visual concepts given edge to provided human prior in terms of augmentation method and schemes. However, the human prior also become inherently weakness for self supervision due to limited understanding about domain and it prevent neural networks to learn representation to their full potential. it imposes more challenges for the vision domains [REFERENCES] e.g. medical imaging, microscopic images, etc. due to limitation of human knowledge to design distorted views by comprehensively compiling the domain specific knowledge. Scarcity of labeled data in medical histopathological domain is already known problem in supervised learning for same reason.\\
%To counter the above stated challenges of human prior and requirement of massive data for self-supervised methods, followings are considerations :
%\begin{itemize}
%    \item Prior/self-supervision signal from data to eventually reduce human prior
%    \item Utilizing learned representation from inter-domain transfer learning in self-supervised pre-training to reduce massive unlabeled data requirement 
%\end{itemize}

%Current work proposes data efficient contrastive similarity based self-supervised approach which focused on data-centred prior. Proposed method, Magnification Prior Contrastive Similarity (MPCS), exploits the magnification prior present in BreakHis data along with utilizes inductive transfer learning from ImageNet source domain. 

 %\subsection{Fine Tuning}
 

==> WACV 2021-MPCS_Arxiv/sections/4_dataset.tex <==
The BreaKHis dataset~\cite{spanhol2016dataset} contains 7909 microscopic histopathology whole slide images (WSI) categorized into benign and malignant classes of breast tumor. WSI is collected from 82 patients, 24 benign and 58 malignant. Images of each patient are provided in four different magnifications 40x, 100x, 200x, and 400x respectively, and their detailed description is mentioned in Table~\ref{tab:experiments_details}. Evaluation metrics suggested in BreakHis~\cite{spanhol2016dataset} and followed by many state-of-the-art methods are \textit{Image-Level Accuracy (ILA)} and \textit{Patient-Level Accuracy (PLA)}. ILA corresponds to the score from the total number of correctly classified images. PLA, also called \textit{Recognition Rate} corresponds to the average image-level accuracy per patient.
This work follows the same evaluation scheme.
Additionally, the cross-magnification evaluation is also performed using both evaluation metrics.


\begin{table}[t]
\caption{Description of BreakHis dataset.}
\label{tab:BreakHis_dataset}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc|c|c}
\hline
                           & \multicolumn{4}{c|}{Magnification}                                                                                                                                                                                       &                         &                           \\
\multirow{-2}{*}{Category} & \multicolumn{1}{c|}{\textbf{40X}}                         & \multicolumn{1}{c|}{\textbf{100X}}                        & \multicolumn{1}{c|}{\textbf{200X}}                        & \textbf{400X}                        & \multirow{-2}{*}{Total} & \multirow{-2}{*}{Patient} \\ \hline
\textbf{Benign}            & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 625}}           & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 644}}           & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 623}}           & {\color[HTML]{1E1E1E} 588}           & 2480                    & 24                        \\
\textbf{Malignant}         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1370}}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1437}}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1390}}          & {\color[HTML]{1E1E1E} 1232}          & 5429                    & {\color[HTML]{444444} 58} \\ \hline
\textbf{Total}             & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{1995}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{2081}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{2013}}} & {\color[HTML]{1E1E1E} \textbf{1820}} & \textbf{7909}           & \textbf{82}               \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/5_experimental_setup.tex <==
This section investigates the representation learning capabilities of the proposed method MPCS on two encoder networks with detailed experimentation on three public datasets.
\subsection{Datasets}
\subsubsection{BreakHis}
BreakHis~\cite{spanhol2016dataset} dataset consists of 2,480 benign and 5,429 malignant histopathological microscopic images from 82 patients at four magnification levels (40×, 100×, 200×, 400×). Each image in the BreakHis dataset is of size 700×460, stained with hematoxylin and eosin (HE). Following the previous works, two evaluation metrics are used, image-level accuracy(ILA) and patient-level accuracy (PLA). PLA shows patient-wise classification performance, calculated as the mean over total no. of patients using patient-score. Patient-score is correctly classified images of the patient over a total number of images of that patient. ILA disregards patient-level details and thus serves as standard image classification accuracy.    
\subsubsection{BACH}
The second dataset, Breast Cancer Histology Images (BACH)~\cite{aresta2019bach} is from the ICIAR2018 Grand Challenge and contains 400 histopathology slides. The BACH dataset has four classes, normal, benign, in-situ, and invasive. The slide size is relatively large, 2048 × 1536 pixels; thus, patches of size 512x512. Two evaluation metrics, patch-wise accuracy and image-wise accuracy, are used, whereas image-wise accuracy is calculated based on majority voting over the patches of the respective image.
\subsubsection{Breast Cancer Cell Dataset}
The third dataset, Breast Cancer Cell Dataset~\cite{gelasca2008evaluation} is from the University of California, Santa Barbara Biosegmentation Benchmark. This dataset contains 58 HE-stained histopathology 896x768 size images of breast tissue, of which 26 are malignant, and 32 are benign. Patches of size 224x224 were created, and image-wise accuracy was calculated using majority voting over patches of the respective image. 
\subsection{Encoder Architectures}
In this current work, the proposed method MPCS investigated two different CNN encoder architectures. ResNet-50~\cite{yu2017dilated} and Efficient-net b2~\cite{tan2019efficientnet} are used for pre-training and fine-tuning. SSL-specific MLP projection head used for Efficient-net b2 is three layers network of 2048-1204-128 units, whereas ResNet-50 is the most common backbone encoder, used projection head adapted from SimCLR, having 1024-128 units. encoder and projection heads are demonstrated in Fig.~\ref{fig:ssl_mpcs}.
\subsection{Training Protocol}
This section shares parameter configurations used in pre-training and fine-tuning. 
\subsubsection{SSL pre-training}
Self-supervised pre-trainings of both encoders take place on the BreakHis dataset for 1000 epochs with temperature parameter $0.01$, learning rate 1e-05, and a set of augmentation methods such as color-jitter, flip, and rotation. Efficient-net b2 encoder pre-trained using Adam optimizer with a batch size of 128 and image input of $(341, 341)$. However, ResNet-50 adapted standard configurations of self-supervised practices and pre-trained using the LARS optimizer with a batch size of 1024 and input image size of 224x224.
\subsubsection{Fine-tuning}
The common training configurations across datasets for both encoders are learning rate of 2e-05, batch size of 32, image input of 224x224, augmentations methods such as random crop, flip, affine, rotation, and color-jitter, and using adam as optimizer. A dropout of 0.3 is used in the fully connected layer.
\subsection{Experimentation Details}
%Several of the works presented in Table \ref{tab:previous_work} use a random 70:30 split of training and test data with repeated trials (\cite{spanhol2016breast, sudharshan2019multiple, gupta2017breast, gupta2018sequential, gupta2019partially}).
%A few other works are ambiguous as to whether full k-fold cross-validation is used or random trials (\cite{patil2019breast, gupta2021breast, benhammou2020breakhis}).
%A careful analysis reveals the downsides of the used data-splitting strategy used in most state-of-the-art methods. However, this strategy performs experiment repetitions over five times; however, it does not endorse the theoretical guarantee for selecting mutually exclusive data points in test-set across the trials because any two consecutive trials are conditionally independent. Thus, generated train and test sets are not mutually exclusive.
%Further, specifically chosen ratio of 70:30 for train-test data splits repeated over 5-times forces some data-points to occur in test set with more frequency than others. Lastly, this strategy does not care for class level distribution in each trial which becomes critical for evaluating class imbalance and small-scale detests.

%A careful analysis reveals the downsides of the data-splitting strategy used in most state-of-the-art methods.
%While this strategy performs experiment repetitions over five times, it does not endorse the theoretical guarantee for selecting mutually exclusive data points in the test-set across the trials (any two trials are conditionally independent). 
%Moreover, the specifically chosen ratio of 70:30 for train-test data splits repeated over 5-times forces some data points to occur in a test set more frequently than others. Lastly, this strategy does not care for class level distribution in each trial which becomes critical for evaluating class imbalance and small-scale detests.

%As also mentioned in Section~\ref{related_work}, A careful analysis reveals downsides of used data-splitting strategy used is most of the state-of-the-art methods. Although, this strategy performs experiment repetitions over 5 times however it does not endorse  theoretical guarantee for selection of mutually exclusive data-points in test set across the trials because any two consecutive trials are conditionally independent. Thus, generated train and test sets are not mutually exclusive. Further, Specifically chosen ratio of 70:30 for train-test data splits repeated over 5-times forces some data-points to occur in test set with more frequency than others. Lastly, this strategy does not care for class level distribution in each trial which becomes critical for evaluation of class imbalance ans small-scale detests.


\begin{comment}
As also mentioned in Section~\ref{related_work} careful analysis shows the following weakness in mentioned data-split strategy:
\begin{enumerate}
    \item The stated data-split strategy does not have any mechanism to ensure the correctness of mean performance evaluation where contribution made by each data-point is ensured in equal or at least in one trial of experiment out of 5. The same is applicable to learning capacity.
    \item The stated strategy does not have any mechanism to reflect the data distribution of imbalanced classes during data-split in each trial out of 5. 
\end{enumerate}
The reasons behind the weakness of 1) and 2) are the following:
\begin{itemize}
    \item Repeated yet any independent random trial of data-splits does not endorse theoretical guarantee for selection of mutually exclusive data-points in the test set across the trials because any two consecutive trials are conditionally independent.
    \item Specifically chosen ratio of 70:30 for train-test data splits repeated over 5-times forces some data-points to occur in the test set with more frequency than others.
\end{itemize}
To cater above-stated issues in the experimentation strategy of dataset division, an improved strategy needs to be formulated which can guarantee the following two aspects:
\begin{enumerate}
    \item Mean performance calculation must be contributed by every data-point of the dataset in an equal amount of participation.
    \item Skewed data distribution due to class imbalances must reflect in every test set from each trial to get real-world agnostic performance (more malignant cases than benign in the dataset).
\end{enumerate}
\end{comment}

To ensure the reliability and consistency of the models, this work follows 5-cross validation data split scheme. This is applied to all three datasets in which each fold contained 20\% data, following class distribution from whole data. Four out of five folds are used for training \& validation, and the remaining one for testing. Thus all the results reported are in terms of mean value with standard deviation.
In the above-stated 5-cross validation settings, both backbone encoders, ResNet-50 and Efficient-net b2, are being pre-trained on the first dataset BreakHis with all three variants (ordered pair, random pair, and fixed pair) of the proposed SSL method MPCS for learning domain-specific representations. Further, downstream-task-specific fine-tuning experiments are carried out to investigate the impact of learned representations for all three datasets e.g., BreakHis, BACH, and Breast Cancer Cell. 
Following are the details of experimentation for each dataset.
Table~\ref{tab:experiments_details} describes fine-tuning experiments for the first dataset BreakHis. All the mentioned experiments for malignancy classification are conducted for both encoders, Efficient-net b2 and ResNet-50 for all four magnifications (40X, 100X, 200X, and 400X). Experiments (Exp-1 to Exp-4) in \textit{Limited Labeled Data Setting} evaluate model performance while using only 20\% labels, whereas experiments (Exp-5 to Exp-8) in \textit{Fully Supervised Setting} use all labels. The sole objective is to compare the performance of models pre-trained on proposed MPCS methods against ImageNet~\cite{deng2009imagenet} pre-trained model to analyze the effect of learned representations. Preferred names in discussion used as MPCS-X for ImageNet $\to$ MPCS-X.
Experiments(Exp-9 to Exp-12) for the second dataset BACH~\cite{aresta2019bach} are described in Table~\ref{tab:exp_bach} based on the ResNet-50 encoder. All the images are divided into 512X512 size patches; thus, performance is measured patch-wise and image-wise (using majority voting suggested in~\cite{vesal2018classification}). The major objectives are 1) evaluating pre-trained models from the proposed method against the ImageNet-based transfer learning approach~\cite{aresta2019bach} 2) evaluating the ability to learn downstream tasks with limited labels ranging from 5\% to 100\% of labels from the train data portion.
Finally, to evaluate the effect of learned domain-specific representations on small-scale data, a series of fine-tuning (all layers trained) and linear evaluation experiments (only fully-connected layers trainable) Exp-13 to Exp-16 are conducted Breast Cancer Cell dataset and described in Table~\ref{tab:exp_bisque}. Similar to BACH dataset, images for this dataset were also divided into sizes 224X224 for training and test, and performance was measured likewise.
%This work designs extensive experimentation mentioned in Table ~\ref{tab:experiments_details} to investigate proposed methods.
%The proposed method compares with the ImageNet supervised transfer learning approach and other state-of-the-art methods over malignancy classification.
%As general rule, all the proposed pre-training methods initializes by ImageNet~\cite{deng2009imagenet} , are mentioned in Table~\ref{tab:experiments_details} as ImageNet $\to$ MPCS-X. However, preferred names in discussion used as MPCS-X.
%All the experiments uses the Efficient-net b2~\cite{tan2019efficientnet} architecture which was chosen based on the trade-off between model complexity and performance based on empirical analysis.
%Experiments in \textit{Limited Labeled Data Setting} (Table~\ref{tab:experiments_details}) uses only 20\% labeled data for fine-tuning and 20\% for testing. Experiments in \textit{Fully Supervised Setting} (Table~\ref{tab:experiments_details}) uses 80\% labeled data for fine-tuning and 20\% for testing to evaluate performance as supervised learning to perform extensive comparison with previous work.
%Current work only focuses on methodological development thus %as mentioned in section~\ref{methdology} however proposed methods are open to adapt different networks, optimizations, data balancing \& augmentation approaches, and domain specific operations to obtain further improved results. Thus, for the aforementioned stated reason, we compare% comparison is performed with all other the state-of-the-art methods and excludes the work which incorporates i) fusion of two or more models \& ensembles approaches, ii) task specific optimized architectures, and iii) methods evaluated on different without or very different data folds although comparison includes previous works on data-split strategy of 70:30, repeated over 5-times.Due to non-availability of fold-wise result details on previous work, statistical significance evaluation is not calculated.
%This work only focuses on methodological development. Thus, the comparison is performed with all other state-of-the-art methods, excluding which incorporates i) fusion of two or more models \& ensembles approach, ii) task-specific optimized architectures, and iii) methods evaluated on very different data folds.
%Although comparison includes previous works on the data-split strategy of 70:30, repeated over 5-times. Statistical significance was calculated to the proposed method and ImageNet approach in the limited labeled data setting; however, it does not take-place for a fully supervised setting due to the non-availability of fold-wise results on other previous work.



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Experiment details for BreakHis dataset}
\vspace{-0.3cm}
\label{tab:experiments_details}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{No.}} & \multicolumn{1}{c|}{\multirow{2}{*}{Pre-training Method}}          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BreakHis data\\  (\%)for SSL\end{tabular}}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Finetuning on \\ BreakHis Dataset\end{tabular}} \\ \cline{4-5} 
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                                              & \multicolumn{1}{c|}{}                                                                                      & \multicolumn{1}{c|}{Train (\%)}                          & Test (\%)                          \\ \hline
\multicolumn{5}{c}{Limited Labeled Data Setting}                                                                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{c|}{Exp-1}                      & \multicolumn{1}{c|}{ImageNet}                                      & \multicolumn{1}{c|}{-}                                                                                     & \multicolumn{1}{c|}{20\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-2}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Fixed Pair}   & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{20\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-3}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Ordered Pair} & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{20\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-4}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Random Pair}  & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{20\%}                                & 20\%                               \\ \hline
\multicolumn{5}{c}{Fully Supervised Data Setting}                                                                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{c|}{Exp-5}                      & \multicolumn{1}{c|}{ImageNet}                                      & \multicolumn{1}{c|}{-}                                                                                     & \multicolumn{1}{c|}{80\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-6}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Fixed Pair} & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{80\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-7}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Ordered Pair}  & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{80\%}                                & 20\%                               \\
\multicolumn{1}{c|}{Exp-8}                      & \multicolumn{1}{c|}{ImageNet $\to$ MPCS-Random Pair}  & \multicolumn{1}{c|}{60\%}                                                                                  & \multicolumn{1}{c|}{80\%}                                & 20\%                               \\ \hline
\end{tabular}%
}
\vspace{-2mm}
\end{table}

\begin{table}[t]
\caption{Experiment details for BACH dataset}
\label{tab:exp_bach}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|cc}
\hline
                      &                                                                                          & \multicolumn{2}{c}{Fine-tuning on BACH dataset}                                                                   \\ \cline{3-4} 
\multirow{-2}{*}{No.} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-training \\ method/weights\end{tabular}} & \multicolumn{1}{c|}{Labels(\%) from Train Data}                                                 & Test data (\%)              \\ \hline
Exp-9                 & ImageNet~\cite{vesal2018classification}-re-implement                                                                                 & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 100\% (~80\% train data)}}                                    & {\color[HTML]{1E1E1E} 20\%} \\
Exp-10                & MPCS-Fixed Pair (BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%, 100\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\
Exp-11                & MPCS-Ordered Pair(BreakHis)                                                              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%, 100\%{]}}} & 20\%                        \\
Exp-12                & MPCS-Random Pair(BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%, 100\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\end{table}


\begin{table}[t]
\caption{Experiment details for Breast Cancer Cell Dataset}
\label{tab:exp_bisque}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|cc|cc}
\hline
                      &                                                                                          & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Fine-tuning on \\ Breast Cancer Cell Dataset\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Linear-evaluation on  \\ Breast Cancer Cell Dataset\end{tabular}} \\ \cline{3-6} 
\multirow{-2}{*}{No.} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-training \\ method/weights\end{tabular}} & \multicolumn{1}{c|}{Train data(\%)}                            & Test data (\%)                           & \multicolumn{1}{c|}{Train data(\%)}                            & \multicolumn{1}{l}{Test data(\%)}              \\ \hline
Exp-13                & MPCS-Fixed Pair (BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & {\color[HTML]{1E1E1E} 20\%}              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & {\color[HTML]{1E1E1E} 20\%}                    \\
Exp-14                & MPCS-Ordered Pair(BreakHis)                                                              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & 20\%                                     & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & 20\%                                           \\
Exp-15                & MPCS-Random Pair(BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & {\color[HTML]{1E1E1E} 20\%}              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}               & {\color[HTML]{1E1E1E} 20\%}                    \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/6_result_discussion.tex <==

\input{sections/tables/evaluation_FT20} 

%\input{sections/tables/evaluation_FT80} \label{ft_80}

\input{sections/tables/evaluation_comparision} 
\input{sections/tables/bach_sota_compare}
\input{sections/tables/bach_results_label_wise}
\input{sections/tables/bisque_sota_compare}

%\input{sections/tables/trained_cross_magnification}

%\input{sections/tables/eval_cross_magnification}
%This work evaluates MPCS which leverages a magnification prior in histopathology images and employs a reduced human prior by providing more degrees of freedom. The results show that this method is beneficial for self-supervised pre-training.
%Table~\ref{ft_20} compares the malignancy classification models fine-tuned on representations learned with and without MPCS pre-training methods in a limited labeled data setting when only 20\% labels are used based on experiments Exp-1 to Exp-4 in Table~\ref{tab:experiments_details}.
The quantitative results and qualitative analysis from extensive experiments on three datasets validate the efficiency of learned representations for the proposed self-supervised pre-training method MPCS. Preliminary investigation on data prior also supports the hypothesis of reducing human prior in self-supervised representation learning.

Results on BreakHis dataset for the experiments Exp-1 to Exp-4 in Table~\ref{tab:experiments_details}  in limited labels setting (20\% labels only) are described in Table~\ref{ft_20}. It shows that all the variants (ordered pair, random pair, and fixed pair) of MPCS pre-trained models obtain significant \textit{(across magnification, p \textless 0.05)} improvement (1.55 $\sim$ 2.52)\% over the ImageNet transfer learning model for all four magnifications and results are competitive with other state-of-the-art methods that have been trained in the fully supervised setting using all labels. Further, Table~\ref{ft_80_sota} compares the performance of experiments Exp-5 to Exp-8 in Table~\ref{tab:experiments_details} in the fully supervised setting (using all labels). The MPCS pre-trained models outperform several state-of-the-art methods with (3.5 $\sim$ 8.0)\% higher accuracy in malignancy classification. Both encoder architectures, Efficient-net b2 and ResNet-50 perform consistently. The t-SNE visualization of the pre-trained ResNet-50 encoder in Figure~\ref{fig:tsne} and class activation maps (CAM)~\cite{selvaraju2017grad} in Figure~\ref{fig:cam_breakhis} show robust representation learning in the pre-tuning and fine-tuning phases, respectively. Additionally, cross-magnification evaluation is also performed as suggested in previous work~\cite{gupta2017breast} and \cite{sikaroudi2021magnification}, results support performance generalization across magnifications, and results can be found in the supplementary material.
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.9\linewidth]{sections/figures/BreakHis_OP.jpg}
    \caption{Comparing CAM from ImageNet and MPCS-OP on BreakHis dataset. Only OP variant CAM is shown for space constraint. Activation - red (darker) color}
    \label{fig:cam_breakhis}
    \vspace{-6mm}
\end{figure}
MPCS pre-trained ResNet-50 models on the BreakHis dataset are further evaluated on two additional datasets. Results on the BACH dataset for the experiments Exp-9 to Exp-12 in Table~\ref{tab:exp_bach} are described in Table~\ref{tab:bach_results_sota_compare} and ~\ref{tab:bach_results_labelwise}. Results in Table~\ref{tab:bach_results_sota_compare} show the performance improvement on four-class classification on image-wise and patch-wise accuracy while comparing with other state-of-the-arts for the ResNet-50 encoder and other architectures. Specifically, compared with other recent work based on contrastive learning-based self-supervised method DPCL~\cite{ciga2022self}, the proposed method MPCS consistently outperforms over a varying range of label usage as shown in Figure~\ref{fig:ssl_dpcl} and obtains an improvement of 4.85\% when using 100\% labels. To compare with ImageNet pre-trained ResNet-50 encoder in identical settings, the method suggested in~\cite{vesal2018classification} is re-implemented and results are reported in Table~\ref{tab:bach_results_sota_compare} for comparison and qualitative analysis through CAM is also shown for samples from the BACH dataset in Figure~\ref{fig:cam_bach}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.9\linewidth]{sections/figures/BACH_ALL_PAIR.png}
    \caption{CAM from ImageNet and MPCS-RP, OP, FP on BACH dataset (MPCS specifically learns to prevent activation on cells present on normal class images).}
    \label{fig:cam_bach}
    \vspace{-6mm}
\end{figure}
Results on the third Breast Cell Cancer dataset for experiments Exp-13 to Exp-15 from Table~\ref{tab:exp_bisque} are compared with other methods in Table~\ref{tab:bisque_results_sota_compare}, shows significant improvement over other methods and obtains 98.18\% in fine-tuning and 96.36\% in linear evaluation. CAM in Figure~\ref{fig:cam_bisque} also supports the method qualitatively. Reproducible source code for all the results reported is added in supplementary content and shall be made available on GitHub. 
\begin{figure}[!ht]
    \centering
    \includegraphics[width =\linewidth]{sections/figures/BISQUE_ALL_PAIR.png}
    \caption{Comparing CAM among MPCS-RP, OP, and FP on Breast Cancer Cell dataset. Activation - red (darker) color}
    \label{fig:cam_bisque}
    \vspace{-6mm}
\end{figure}
%The t-SNE visualization in Figure~\ref{fig:tsne} of test set shows concrete segregated groups supporting robust representation learning even without fine-tuning on labels pretrained ResNet-50 encoder shows

%Results on BreakHis dataset for the experiments Exp-1 to Exp-4 in Table~\ref{tab:experiments_details}  in limited labels setting in Table~\ref{ft_20} when pretrained model fine-tuned on only 20\% labels  Table~\ref{ft_20} compares the performance of Exp-1 to Exp-4 in Table~\ref{tab:experiments_details} where only 20\% of the labeled data is used for supervised fine-tuning. 
%Results compete with fully supervised learning malignancy classification state-of-the-art performance and obtains significant (across magnification, p \textless 0.05) improvement (1.55 $\sim$ 2.52)\% over the ImageNet transfer learning method for all four magnifications showing label efficiency.
%The MPCS pre-trained models obtain significant \textit{(across magnification, p \textless 0.05)} improvement (1.55 $\sim$ 2.52)\% over the ImageNet transfer learning method for all four magnifications showing label efficiency.
%Additionally, the results are competitive with state-of-the-art methods that have been trained with 70\%-80\% labeled data.


%Table~\ref{ft_80_sota} compares the performance of Exp-5 to Exp-8 in Table~\ref{tab:experiments_details} where 80\% of the labeled data is used for supervised fine-tuning.
%Additionally, the table shows the previous works on the dataset.
%The MPCS pre-trained models obtain higher accuracy than the ImageNet transfer learning method for all magnification levels and are competitive with state-of-the-art methods, outperforming the several methods with (3.5 $\sim$ 8.0)\% higher accuracy in malignancy classification.
%Also, following the experiments Exp-5 to Exp-7 in Table~\ref{tab:experiments_details} in fully supervised learning setting, Table~\ref{ft_80} shows improved performance over ImageNet transfer learning method and Table~\ref{ft_80_sota} compares with other state-of-the-art methods showing (3.5 $\sim$ 8.0)\% higher accuracy in malignancy classification.

%Further, Table~\ref{x_mag_type1} and \ref{x_mag_type2} shows proposed MPCS is magnification invariant than transfer learning method in cross-magnification performance comparison.    

%Proposed self-supervised pre-training methods, Ordered Pair and Random Pair evaluated on downstream task of detection of malignancy. Besides, limited labeled data settings, also evaluated in fully supervised settings to extensively compare with most of the previous methods benchmarked on BreakHis\cite{spanhol2016dataset} having single model approach belongs deep learning and conventional methods. Referring Table \ref{tab:result_pla_ft80}, our proposed methods outperforms on against all stated previous methods on all four magnification and mean value, obtains of mean patient level accuracy $91.63\%$ and $92.15\%$ respectively.

\subsection{Self-supervised method MPCS demonstrates label efficiency}

\begin{figure}[t]
    \centering
    \includegraphics[width =0.6\linewidth]{sections/figures/SSL_label_wise_compare_bach.png}
    \caption{Comparison with DPCL~\cite{ciga2022self} for label efficiency on classification task on BACH dataset}
    \label{fig:ssl_dpcl}
    \vspace{-7mm}
\end{figure}
%preforms well with less labels
%\todo - Refers results for limited labeled data settings to show cases about obtaining the sota results with 20\% labels, better than Image-net transfer learning - important to showcases - results are statistically significant across magnification to reject null hypothesis.]
%To investigate the capabilities of self-supervised pre-training for label efficiency, current work fine-tune the ImageNet pre-trained EffcientNet b2 model on 20\% labeled data of BreakHis~\cite{spanhol2016dataset} to compare with all three variants of self-supervised MPCS pre-trained models mentioned in Table~\ref{tab:experiments_details}  for all four (40x, 100x, 200x, and 400x) magnifications. 
All three variants of the proposed method MPCS demonstrate label efficiency on downstream tasks. Results in Table~\ref{ft_20} On BreakHis dataset, MPCS fine-tuned models obtain (significant improvement p \textless 0.01) proportionally bigger margins of improvement of (2.52±0.02)\% over ImageNet pre-trained model while only 20 \% labels are used for all magnification scales. These results match the performance of other state-of-the-art methods mentioned in Table~\ref{ft_80_sota} which have been trained on 100\% labels. Following the trend, MPCS pre-trained models consistently outperform on the BACH dataset compared with the recent contrastive learning-based method DPCL~\cite{ciga2022self} in a complete range of labels from 5\% to 100\%, shown in Figure~\ref{fig:ssl_dpcl}. 
%The first observation from the results in Table~\ref{ft_20} showcases 
%that self-supervised method, MPCS obtains proportionally bigger margins when fine-tuning with fewer labels that are only 20\%.
%All the variant of proposed self-supervised models outperforms significantly (across magnification, p \textless 0.05) over the ImageNet transfer learning model on all the magnification factors (40x, 100x, 200x, and 400x) for both evaluation criteria.
%Specifically, the MPCS-Ordered Pair method demonstrates robust representation learning capability during fine-tuning in limited labeled data setting (20\% labels) with (2.52±0.02)\% significant improvement(p \textless 0.01) in patient-level accuracy and similar results on image-level accuracy over ImageNet model.
%It matches the performance to the mentioned state-of-the-art methods from the fully supervised learning setting in Table~\ref{ft_80_sota} for both evaluations.
%Further, a noticeable fact is that MPCS pre-trained models are outperforming the ImageNet model for a larger fraction of labels in a fully supervised learning setting, as shown in Table~\ref{ft_80_sota}.

%the potential about  of self-supervised models to generalizes when fine-tuned on only 20\% labels.

%First, we observe that pretraining using self-supervised models can significantly help with label efficiency for medical image classification, and in all of the fractions, self-supervised models outperform the supervised baseline. Moreover, these results suggest that MICLe yields proportionally larger gains when fine-tuning with fewer labeled examples. In fact, MICLe is able to match baselines using only 20% of the training data for ResNet-50 (4×) and 30% of the training data for ResNet152 (2×). Results on the CheXpert dataset are included in

\subsection{Data prior enables self-supervision on small-scale datasets}
%Self-supervised learning methods (\cite{chen2020simple}, ~\cite{he2020momentum}, \cite{chen2021exploring}, \& \cite{grill2020bootstrap}) in the computer vision domain often use millions of images from ImageNet~\cite{deng2009imagenet} to learn.
The proposed MPCS method enables self-supervised representation learning on the small-scale dataset by extensively using a data prior (supervision signal from data) e.g. magnification factors (40X, 100X, 200X, and 400x). It decreases the dependence on human-curated priors e.g. augmentation method choices during self-supervised pre-training.  
%However, the model evaluated in this work still used the large-scale data through inductive transfer learning of Efficient-net b2 parameters pre-trained on ImageNet, which further helps to scale pre-training.
% from the small-scale data of the downstream task itself.
%The self-supervised learning methods on natural visual concept domains (i.e. PIRL~\cite{misra2020self},  SimCLR~\cite{chen2020simple}, MoCo~\cite{he2020momentum}), BYOL~\cite{grill2020bootstrap}, \& SimSiam~\cite{chen2021exploring}) are pre-trained on millions of images from ImageNet~\cite{deng2009imagenet} dataset.
%However, the MPCS self-supervised method focused on supervision signal from data itself (i.e. magnification).
%The magnification factor is exploited for pair generation of views from the input image by integrating it with human prior.
%Further, inductive transfer was employed to initialize model parameter with supervised ImageNet pre-trained Efficient-net model parameters.
%Using a magnification prior from data and inductive transfer enables self-supervised representation learning on small-scale BreakHis~\cite{spanhol2016dataset} dataset, which obtains patient-level accuracy 88.77\% and 92.15\% in limited labeled data and fully supervised learning settings, respectively.
\subsection{MPCS learns robust self-supervised representations}
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.8\linewidth]{sections/figures/tsne_all_pair.png}
    \caption{tsne-visualization of the features from MPCS model (on BreakHis) without fine-tuning. Blue(benign); red(malignant).  }
    \label{fig:tsne}
    \vspace{-4mm}
\end{figure}
Explicitly focusing on the robustness of learned representations, Figure~\ref{fig:tsne} strongly supports the fact that MPCS pre-trained models can capture and learn discriminative features across the classes during the self-supervised pre-training phase itself without knowing about actual human-provided labels. It is worth mentioning that data points of different classes are easily separable by either linear or non-linear boundaries for all four magnifications for all variants of the MPCS method. The CAM of fine-tuned models depicted in Figures~\ref{fig:cam_breakhis} and ~\ref{fig:cam_bach} also indicate that MPCS pre-trained models activate regions of interest (dark red colors show strong activation) more efficiently than the ImageNet pre-trained model for BreakHis and BACH datasets.  
\subsection{Preliminary support for the hypothesis  about reducing human inducted priors}
The MPCS-Ordered Pair inducts weaker human-prior in pair sampling. Thus, the MPCS method obtains one DoF for randomly choosing the first input view. In comparison, the MPCS-Fixed Pair, which inducts stronger human prior by choosing both views, 200x and 400x by human-prior, gives zero DoF to the MPCS method. The MPCS-Random Pair, in which the MPCS method obtains the highest degree of freedom since the human-prior is absent.
\begin{figure}[!ht]
    \centering
    \includegraphics[width =0.6\linewidth]{sections/figures/degree_of_freedom_ILA_PLA_extended.png}
    \caption{Comparison for human priors - Indicates weaker human-prior(moderate DoF for method) outperforms stronger and no human-prior during limited (20\% labels) data\\}
    \label{fig:degree_of_freedom_ILA_PLA}
    \vspace{-8mm}
\end{figure}
%The result in Table~\ref{ft_20} shows MPCS-Ordered Pair gains improvement over MPCS-Fixed Pair with ILA of 0.77 and PLA of 0.72. Similarly, MPCS-Ordered Pair improves over MPCS-Random Pair with ILA of 0.73 and PLA of 0.66.
%over MPCS-Fixed Pair and 0.73 over MPCS-Random Pair.
%Need to re-write - Comparisons shows MPCS-Ordered Pair achieves higher accuracy for all the magnification factors with mean image and patient-level accuracy improvement of 0.73\% and 0.66\%   (Refer Table~\ref{ft_20}).
Figure~\ref{fig:degree_of_freedom_ILA_PLA} explains the trends when fewer labels are used, that both encoders that weaker human-prior based pair sampling tends to outperform over extreme cases of stronger human prior or the absence of it. However, it requires detailed explorations of different datasets and tasks. Similar patterns were also observed on the BACH dataset that the ordered pair outperforms over other two variants.
%\subsection{Comparing the proposed method with other state-of-the-art methods}
%MPCS demonstrates outstanding performance on BreakHis for both the 20\% and 80\% labeled data cases.
%Table~\ref{ft_80_sota} compares the proposed method MPCS-Ordered Pair and MPCS-Random Pair extensively with previous works on image and patient level accuracy and highlights the top two results for each.
%Table~\ref{ft_80_sota} compares MPCS with previous works on image and patient-level accuracy and highlights the top two results for each.
%The top two mean patient-level accuracies are 92.15\% and 91.63\%, which are obtained by MPCS-Random Pair and MPCS-Ordered Pair respectively, and it shows improvement of 3.51\% and 2.99\% over previous best results SMSE~\cite{sun2021magnificationindependent} in Table~\ref{ft_80_sota}.
%Similarly, Top two mean image-level accuracies are 92.23\% and 91.94\%, which are obtained by MPCS-Random Pair and MPCS-Ordered Pair, respectively, and it shows improvement of 3.83\% and 3.54\% over previous best results SMSE~\cite{sun2021magnificationindependent}.
%MPCS-Random Pair and MPCS-Ordered Pair achieves the top two results for both image and patient-level images when averaged across magnifications, with around three percentage points increase above the previous best results~\cite{sun2021magnificationindependent}.
%Considering magnification specific performances, MPCS-Ordered Pair and Random Pair consistently obtains top two ranks except for patient-level accuracy at 400x, and image-level accuracy at 40x are included GLPB~\cite{ataky2020data} and RPDB~\cite{man2020classification} within the top two results.
%As for magnification-specific performance, Ordered Pair and Random Pair achieve the top two results in all but two categories and get the top results in all but one.
%It is also worth mentioning that results for other works which do not follow repeated folds and obtain higher accuracy, some specific fold results for MPCS-Ordered Pair and MPCS-Random Pair also obtains PLA 98.82\% and 96.99\% respectively.
%\todo - Compare proposed the methods for degree of freedom. refer results in %Table ~\ref{tab:results_ft20}, refer diagram \ref{fig:degree_of_freedom_ILA_PLA} to prove hypothesis in method section
%As hypothesized in ~\ref{ssl} that increased human inducted priors which also imposes limitation due to  reduces the degree of freedom for self-supervised method which prevents representation learning at full potential
%Section~\ref{ssl} hypothesized i) Imposing human knowledge of concepts strongly in terms of human prior, reduces the degree of freedom for self-supervised methods which prevents representation learning at full potential ii) Current state of self-supervised learning relies on multiple distorted views of input visual thus requires human prior for transformations/augmentations. So effectively, a more balanced approach of human inducted prior is essential. Three strategies of inducted human prior were formulated (refer Figure~\ref{fig:degrre_of_freedom} and ~\ref{fig:human_prior}) depicting stronger to no prior for detailed investigation. An empirical analysis conducted on degree of freedom and downstream task performance for self-supervised methods exploiting results on limited labeled data setting. Referring to visual explanation in  Stronger human prior represented by Fixed Pair method and no human prior represented by Random Pair method comparatively remains under-performing for classification task against the optimally managed human prior method Order Pair.
%\subsection{Self-supervised methods learns magnification invariant representations}
%\todo - Refer Table ~\ref{tab:results_ft80_cross_magnificaiton_type2} and Table ~\ref{tab:results_ft80_cross_magnificaiton} and make statement.
%MPCS methods not only outperforms for magnification specific task stated in Table~\ref{ft_20} and ~\ref{ft_80} but representations learned through proposed method also demonstrate consistent edge in classification performance in cross-magnification evaluation over ImageNet model. Table~\ref{x_mag_type1} shows (type-1 mean cross magnification evaluation) mean cross-magnification accuracy where the model is evaluated on other magnifications except the magnification on which model was trained. The MPCS-Order Pair methods outperform the ImageNet model and other methods with mean cross-magnification ILA 80.99\% and PLA 81.49\% when model trained on 40x magnification and evaluated on 100x, 200x, and 400x. Whereas MPCS-Random Pair outperforms with mean cross-magnification ILA 84.84\% and PLA 82.97\% when trained on 200x and ILA 84.83\% and PLA 83.76\% when trained on 400x. For 100x, MPCS-Ordered Pair obtains ILA 80.99\%, and MPCS-Random Pair obtains PLA 85.05\%. Further Table~\ref{x_mag_type2} evaluates the mean performance of models trained on other magnifications except on which evaluation is performed (type-2 mean cross magnification evaluation). Interestingly, type-2 cross magnification evaluation also shows similar trends except in 400x, in which the ImageNet model obtained high PLA performance. Empirical analysis on type-1 and type-2 cross magnification suggests that MPCS self-supervised pre-trained models perform better than ImageNet by learning magnification invariant representations.         
%\begin{itemize}
%\color{blue}
%\item TODO - Discuss results SOTA comparison for fully supervised setting
%\item TODO - Discuss results limited data setting - obtaining SOTA in 20\% %labeled data
%\item Reasoning - 1) utilizing data signal with minimal prior inducted by human
%\item TODO - Discuss the empirical evidence to support hypothesis made in methodology section of SSL on usage of human prior/degree of freedom referring Figure 2 and 3
%\end{itemize}

%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width =0.8\linewidth]{sections/figures/PLA_DoF.png}
%    \caption{Relation between Degree of Freedom (Human Prior) of self-supervised  methods and Patient %Level Accuracy across fine-tuned on 20\% labeled data}
%    \label{fig:degree_of_freedom_PLA}
%\end{figure}




%thus we only exclude work in comparisons which are related to fusion based methods \cite{deniz2018transfer} and \cite{gupta2018sequential} having multiple machine learning approaches together, ensemble approaches \cite{gupta2017breast}, and methods evaluated on different data folds or without repeated fold, \cite{gupta2021breast}, \cite{benhammou2020breakhis}. Referring Table \ref{tab:result_pla_ft80}, our proposed methods outperforms on against all stated previous work on all four magnification and mean value, obtains of patient level accuracy $91.63\%$ and $92.15\%$ respectively.



==> WACV 2021-MPCS_Arxiv/sections/7_conclusion_future_work.tex <==
%This work proposed a novel self-supervised pre-training method, Magnification Prior Contrastive Similarity which enables self-supervised pre-training for comparatively small-scale breast cancer microscopic image dataset BreakHis~\cite{spanhol2016dataset} for efficient representation learning by exploiting supervision signals from data.
The novel MPCS method enables self-supervised pre-training for comparatively small-scale breast cancer microscopic image dataset BreakHis~\cite{spanhol2016dataset} for efficient representation learning by exploiting supervision signals from data.
Results on three public datasets have confirmed the excellence of the MPCS method. MPCS learns better representations by exploiting magnification priors (OP is best among all) and distinguishing among different cells in downstream tasks. It could be better to investigate on a continuous scale of magnification scales considered in this paper. In the future, we intend to investigate magnification prior to other self-supervised learning approaches focusing on redundancy reduction and Siamese networks.


%Following are the main contributions:
% \begin{itemize}
% \item Enables self-supervised learning on small-scale histopathology dataset by exploiting data prior and transfer learning
% \item Demonstrate label efficient self-supervised learning method and obtains state-of-the-art performance only on 20\% labels data
% \item Outperforming malignancy classification performance over previous works by 3.51\% in fully supervised learning setting 
% \item Establishes relation between human inducted prior and representation learning potential for self-supervised method. Empirically proves the fact that reducing human prior leads to efficient representation learning
% \item Empirical evidence on cross-magnification evaluation to demonstrate magnification invariant representation learning
% \end{itemize}
%Future plan for proposed work include investigation and extension of the proposed methods towards multiple downstream tasks, cross-domain adaptation, incorporation of unsupervised and self-supervised transfer learning, and focus on further reducing the human prior. Also, aim to investigate other joint embedding architecture \& method based approaches including distillation and information maximization.
%Also, aim to investigate other joint embedding architecture \& method based approaches including distillation and information maximization.
%Future work includes investigating on cross-domain adaptation, utilizing unsupervised and self-supervised transfer learning, and detailed validation on the human-prior hypothesis.
% Contribution
\begin{comment}
\begin{itemize}
    \color{blue}
    \item TODO - explored self supervised paradigm on histopathlogical images in general , specifically on BreakHis
    \item TODO - Presented SSL method which works on small scale dataset by emphasizes on reducing human prior and by exploit data signals from data, using inductive transfer from image-net.
     1. obtains SOTA only on 20\% labeled data
     2. Outperforms previous SOTA i n fully supervised setting
     3. Cross magnifications performance - out of distribution generalization
     \item TODO -Empirical evidence on effect of inducted human prior on potential of network's learning 
\end{itemize}
Future work
\begin{itemize}
\color{blue}
\color{blue}
    \item TODO - Investigation on domain adaptation, additional down stream tasks, Further exploration to reduce human prior in SSL in contrastive and other ssl paradigm,Focusing other architectural alternatives, training protocol, incorporating unsupervised and self-supervised transfer learning possibilities from imagenet and other domains. 
\end{itemize}
\end{comment}



==> WACV 2021-MPCS_Arxiv/sections/tables/bach_results_label_wise.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\caption{Performance evaluation (image-wise accuracy and f1 score) of proposed method MPCS on BACH dataset for limited label range for ResNet-50 encoder.}
\label{tab:bach_results_labelwise}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\hline
\begin{tabular}[c]{@{}c@{}}Label(\%) from\\ train data\end{tabular} & \multicolumn{3}{c|}{F1 score (test data)}                                                              & \multicolumn{3}{c}{Accuracy (test data)}                                                                  \\ \hline
                                                                    & MPCS-FP                          & MPCS-OP                          & MPCS-RP                          & MPCS-FP                           & MPCS-OP                           & MPCS-RP                           \\ \hline
5\%                                                                 & {\color[HTML]{1E1E1E} 0.50±0.05} & {\color[HTML]{1E1E1E} 0.50±0.05} & {\color[HTML]{1E1E1E} 0.51±0.05} & {\color[HTML]{1E1E1E} 51.25±5.02} & {\color[HTML]{1E1E1E} 50.00±4.80} & {\color[HTML]{1E1E1E} 53.00±5.06} \\
10\%                                                                & {\color[HTML]{1E1E1E} 0.60±0.05} & {\color[HTML]{1E1E1E} 0.61±0.04} & {\color[HTML]{1E1E1E} 0.61±0.05} & {\color[HTML]{1E1E1E} 60.50±4.88} & {\color[HTML]{1E1E1E} 61.75±3.93} & {\color[HTML]{1E1E1E} 62.50±4.60} \\
20\%                                                                & {\color[HTML]{1E1E1E} 0.65±0.03} & {\color[HTML]{1E1E1E} 0.70±0.04} & {\color[HTML]{1E1E1E} 0.68±0.02} & {\color[HTML]{1E1E1E} 69.25±2.92} & {\color[HTML]{1E1E1E} 71.00±3.90} & {\color[HTML]{1E1E1E} 69.00±2.89} \\
40\%                                                                & {\color[HTML]{1E1E1E} 0.79±0.04} & {\color[HTML]{1E1E1E} 0.81±0.04} & {\color[HTML]{1E1E1E} 0.80±0.03} & {\color[HTML]{1E1E1E} 80.75±3.40} & {\color[HTML]{1E1E1E} 81.75±3.52} & {\color[HTML]{1E1E1E} 81.50±3.05} \\
60\%                                                                & {\color[HTML]{1E1E1E} 0.87±0.03} & {\color[HTML]{1E1E1E} 0.87±0.03} & {\color[HTML]{1E1E1E} 0.86±0.03} & {\color[HTML]{1E1E1E} 87.70±3.48} & {\color[HTML]{1E1E1E} 87.75±3.10} & {\color[HTML]{1E1E1E} 86.50±3.00} \\
80\%                                                                & {\color[HTML]{1E1E1E} 0.89±0.03} & {\color[HTML]{1E1E1E} 0.90±0.02} & {\color[HTML]{1E1E1E} 0.89±0.02} & {\color[HTML]{1E1E1E} 89.25±3.02} & {\color[HTML]{1E1E1E} 90.75±2.17} & {\color[HTML]{1E1E1E} 89.75±0.02} \\
100\%                                                               & {\color[HTML]{1E1E1E} 0.90±0.02} & {\color[HTML]{1E1E1E} 0.91±0.02} & {\color[HTML]{1E1E1E} 0.90±0.02} & {\color[HTML]{1E1E1E} 90.55±2.05} & {\color[HTML]{1E1E1E} 91.85±1.77} & {\color[HTML]{1E1E1E} 91.00±2.32} \\ \hline
\end{tabular}%
}
\vspace{-3mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/bach_sota_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\caption{Performance comparison of proposed method MPCS (ResNet-50 encoder) on BACH dataset with other state-of-the-arts for four class classification. RN-50 indicates ResNet-50.}
\resizebox{\columnwidth}{!}{%
\label{tab:bach_results_sota_compare}
\begin{tabular}{c|cc|cc}
\hline
                                                                & \multicolumn{2}{c|}{Image-wise accuracy}                              & \multicolumn{2}{c}{Patch-wise accuracy}                               \\ \cline{2-5} 
\multirow{-2}{*}{Method}                                        & validation                        & test                              & validation                        & test                              \\ \hline
PT~\cite{roy2019patch}                                                              & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} 90.00}      & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} 77.40}      \\
HN~\cite{yan2020breast} (RN-50)                                                      & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} 81.60}      & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} -}          \\
HN~\cite{yan2020breast}                                                              & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} 91.30}      & {\color[HTML]{1E1E1E} -}          & {\color[HTML]{1E1E1E} 82.10}      \\
DPCL~\cite{ciga2022self}                                                            & -                                 & {\color[HTML]{1E1E1E} 87.00}      & -                                 & -                                 \\
\begin{tabular}[c]{@{}c@{}}ImageNet~\cite{vesal2018classification}\\ re-implement\end{tabular} & {\color[HTML]{1E1E1E} 92.40±2.04} & {\color[HTML]{1E1E1E} 90.50±2.10} & {\color[HTML]{1E1E1E} 80.56±3.06} & {\color[HTML]{1E1E1E} 80.00±2.64} \\
\hline
MPCS-FP                                                         & {\color[HTML]{1E1E1E} 92.50±1.90} & {\color[HTML]{1E1E1E} 90.55±2.05} & {\color[HTML]{1E1E1E} 84.25±1.88} & {\color[HTML]{1E1E1E} 82.79±2.05} \\
MPCS-OP                                                         & {\color[HTML]{1E1E1E} \textbf{93.31±1.85}} & {\color[HTML]{1E1E1E} \textbf{91.85±1.77}} & {\color[HTML]{1E1E1E} \textbf{83.90±1.89}} & {\color[HTML]{1E1E1E} \textbf{83.13±2.00}} \\
MPCS-RP                                                         & {\color[HTML]{1E1E1E} 93.00±1.88} & {\color[HTML]{1E1E1E} 91.00±2.32} & {\color[HTML]{1E1E1E} 83.78±2.09} & {\color[HTML]{1E1E1E} 82.90±2.10} \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/bisque_sota_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\caption{Performance measure of proposed method MPCS (ResNet-50 encoder) on Breast Cancer Cell Dataset}
\resizebox{\columnwidth}{!}{%
\label{tab:bisque_results_sota_compare}
\begin{tabular}{c|cccccc}
\hline
                         & \multicolumn{3}{c}{Fine-tuned}                                                                                                                 & \multicolumn{3}{c}{Linear-evaluation}                                                                                              \\ \cline{2-7} 
\multirow{-2}{*}{Method} & accuracy                                   & precision                                 & \multicolumn{1}{c|}{recall}                           & accuracy                                   & precision                                 & recall                                    \\ \hline
ST~\cite{rezaeilouyeh2016microscopic}                       & {\color[HTML]{1E1E1E} 86.00±3.00}          & {\color[HTML]{1E1E1E} -}                  & \multicolumn{1}{c|}{\textbf{1.0}}                     & {\color[HTML]{1E1E1E} -}                   & {\color[HTML]{1E1E1E} -}                  & -                                         \\
MATN~\cite{konstantinov2022multi}                     & {\color[HTML]{1E1E1E} 91.70}               & {\color[HTML]{1E1E1E} -}                  & \multicolumn{1}{c|}{-}                                & {\color[HTML]{1E1E1E} -}                   & {\color[HTML]{1E1E1E} -}                  & -                                         \\
ATN~\cite{ilse2018attention}                      & {\color[HTML]{1E1E1E} 75.50±1.60}          & {\color[HTML]{1E1E1E} 0.73±0.01}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 0.73±0.04}} & -                                          & -                                         & -                                         \\ \hline
MPCS-FP                  & {\color[HTML]{1E1E1E} 98.14±2.05}          & {\color[HTML]{1E1E1E} 0.99±0.01}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 0.98±0.01}} & {\color[HTML]{1E1E1E} 96.29±1.90}          & {\color[HTML]{1E1E1E} 0.97±0.01}          & {\color[HTML]{1E1E1E} 0.96±0.01}          \\
MPCS-OP                  & {\color[HTML]{1E1E1E} \textbf{98.18±1.80}} & {\color[HTML]{1E1E1E} \textbf{0.99±0.01}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 0.98±0.01}} & {\color[HTML]{1E1E1E} \textbf{96.36±1.88}} & {\color[HTML]{1E1E1E} \textbf{0.97±0.01}} & {\color[HTML]{1E1E1E} \textbf{0.96±0.01}} \\
MPCS-RP                  & {\color[HTML]{1E1E1E} 98.10±2.00}          & {\color[HTML]{1E1E1E} 0.985±0.01}         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 0.98±0.01}} & {\color[HTML]{1E1E1E} 96.22±2.02}          & {\color[HTML]{1E1E1E} 0.965±0.01}         & {\color[HTML]{1E1E1E} 0.96±0.01}          \\ \hline
\end{tabular}%
}
%\vspace{-6mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/eval_cross_magnification.tex <==
\begin{table}[h]
\caption{Type 2 cross magnification performance  comparison of proposed methods (select one magnification in on which model was not trained). The values represent mean performance of a  magnification whereas trained on other magnifications (e.g. evaluated on 40x and trained on 100x, 200x, and 400x.}
%\caption{Comparison of Proposed self-supervised pre-training methods Ordered Pair \& Random Pair with (ImageNet pretrained) Transfer Learning on mean cross-magnification performance (excludes magnification for which model evaluated) in fully supervised setting}
\label{tab:results_ft80_cross_magnificaiton_type2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|llll}
\hline
                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Evaluated \\ on 40X\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Evaluated \\ on 100X\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Evaluated \\ on 200X\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Evaluated \\ on 400X\end{tabular}} \\ \cline{2-5} 
\multirow{-2}{*}{Method} & \multicolumn{4}{c}{Mean Cross-Magnification Image Level Accuracy}                                                                                                                                                                                                                                                                           \\ \hline
ImageNet        & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.33 ±   4.32}}                       & \multicolumn{1}{l|}{{\color[HTML]{444444} 83.65 ±   6.07}}                        & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.31 ±   8.93}}                        & {\color[HTML]{444444} 78.86 ±   10.62}                                           \\
MPCS-Ordered Pair             & \multicolumn{1}{l|}{{\color[HTML]{444444} 85.35 ±   4.29}}                       & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.56 ±   6.06}}                        & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{85.28 ±   8.20}}}               & {\color[HTML]{444444} 78.98 ±   7.82}                                            \\
MPCS-Random Pair              & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{86.55 ±   5.10}}}              & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{84.82 ±   5.54}}}               & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.99 ±   7.79}}                        & {\color[HTML]{444444} \textbf{79.17 ±   9.60}}                                   \\ \hline
\multicolumn{1}{l|}{}    & \multicolumn{4}{c}{Mean Cross-Magnification Patient Level Accuracy}                                                                                                                                                                                                                                                                         \\ \hline
ImageNet        & \multicolumn{1}{l|}{{\color[HTML]{444444} 81.71 ±   6.25}}                       & \multicolumn{1}{l|}{{\color[HTML]{444444} 83.76 ±   6.82}}                        & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.35 ±   8.40}}                        & {\color[HTML]{444444} \textbf{80.33 ±   8.10}}                                   \\
MPCS-Ordered Pair             & \multicolumn{1}{l|}{{\color[HTML]{444444} 81.97 ±   6.25}}                       & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.54 ±   6.52}}                        & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.63 ±   7.80}}                        & {\color[HTML]{444444} 79.51 ±   5.20}                                            \\
MPCS-Random Pair              & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{83.24 ±   6.89}}}              & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{84.98 ±   6.12}}}               & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{84.84 ±   7.04}}}               & {\color[HTML]{444444} 79.92 ±   6.53}                                            \\ \hline
\end{tabular} %
}
\label{x_mag_type2}
%\vspace{-4mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/evaluation_FT20.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\caption{Performance evaluation of the proposed methods in limited labelled data setting when fine-tuning only on 20\% labeled data. (across magnification, p \textless 0.05 for all three self-supervised methods for PLA). Ablation results for 40\%, 60\%, and 80\% labels are provided in supplementary content.}
\label{ft_20}
\begin{scriptsize}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Encoder                            & Metric                                                                              & Method       & 40X                                        & 100X                                       & 200X                                       & 400X                                       & Mean                                                   \\ \hline
                                   &                                                                                     & ImageNet     & {\color[HTML]{1E1E1E} 86.36±6.13}          & {\color[HTML]{1E1E1E} 87.80±4.15}          & {\color[HTML]{1E1E1E} 86.82±5.74}          & {\color[HTML]{1E1E1E} 84.98±6.05}          & 86.49±5.63                                             \\
                                   &                                                                                     & FixedPair    & {\color[HTML]{1E1E1E} 87.26±4.46}          & {\color[HTML]{1E1E1E} 87.45±2.35}          & {\color[HTML]{1E1E1E} 89.38±2.18}          & {\color[HTML]{1E1E1E} 88.12±3.84}          & \multicolumn{1}{l}{{\color[HTML]{444444} 88.05 ±3.20}} \\
                                   &                                                                                     & Ordered Pair & {\color[HTML]{1E1E1E} \textbf{87.40±3.73}} & {\color[HTML]{1E1E1E} \textbf{89.30±2.74}} & {\color[HTML]{1E1E1E} \textbf{90.50±2.19}} & {\color[HTML]{1E1E1E} \textbf{88.35±3.30}} & \textbf{88.89±2.99}                                    \\
                                   & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Image Level \\ Accuracy\end{tabular}}   & Random Pair  & {\color[HTML]{1E1E1E} 86.21±4.20}          & {\color[HTML]{1E1E1E} 89.55±2.84}          & {\color[HTML]{1E1E1E} 89.18±4.05}          & {\color[HTML]{1E1E1E} 87.34±3.44}          & 88.07±3.63                                             \\ \cline{2-8} 
                                   &                                                                                     & ImageNet     & {\color[HTML]{1E1E1E} 86.13±5.15}          & {\color[HTML]{1E1E1E} 87.76±6.03}          & {\color[HTML]{1E1E1E} 85.79±4.10}          & {\color[HTML]{1E1E1E} 85.51±5.27}          & 86.30±5.14                                             \\
                                   &                                                                                     & FixedPair    & {\color[HTML]{1E1E1E} 86.90±4.14}          & {\color[HTML]{1E1E1E} 87.64±3.05}          & {\color[HTML]{1E1E1E} 89.60±3.28}          & {\color[HTML]{1E1E1E} 88.26±3.05}          & \multicolumn{1}{l}{{\color[HTML]{444444} 88.10 ±3.38}} \\
                                   &                                                                                     & Ordered Pair & {\color[HTML]{1E1E1E} \textbf{87.19±3.20}} & {\color[HTML]{1E1E1E} \textbf{88.86±2.58}} & {\color[HTML]{1E1E1E} \textbf{90.20±3.26}} & {\color[HTML]{1E1E1E} \textbf{88.96±3.22}} & \textbf{88.80±3.07}                                    \\
\multirow{-8}{*}{Efficient-net b2} & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Patient Level\\  Accuracy\end{tabular}} & Random Pair  & {\color[HTML]{1E1E1E} 87.17±3.88}          & {\color[HTML]{1E1E1E} 88.36±2.84}          & {\color[HTML]{1E1E1E} 88.58±4.01}          & {\color[HTML]{1E1E1E} 88.66±3.13}          & 88.19±3.48                                             \\ \hline
                                   &                                                                                     & ImageNet     & {\color[HTML]{1E1E1E} 87.40±4.88}          & {\color[HTML]{1E1E1E} 86.22±5.71}          & {\color[HTML]{1E1E1E} 86.02±4.74}          & {\color[HTML]{1E1E1E} 85.30±5.95}          & 86.24±5.32                                             \\
                                   &                                                                                     & FixedPair    & {\color[HTML]{1E1E1E} 86.69±3.96}          & {\color[HTML]{1E1E1E} 86.94±3.05}          & {\color[HTML]{1E1E1E} 88.76±2.28}          & {\color[HTML]{1E1E1E} \textbf{88.81±2.77}} & \multicolumn{1}{l}{{\color[HTML]{444444} 87.68 ±3.01}} \\
                                   &                                                                                     & Ordered Pair & {\color[HTML]{1E1E1E} \textbf{87.56±3.48}} & {\color[HTML]{1E1E1E} \textbf{88.60±3.01}} & {\color[HTML]{1E1E1E} \textbf{89.77±2.19}} & {\color[HTML]{1E1E1E} 87.61±3.48}          & \textbf{88.38±3.04}                                    \\
                                   & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Image Level \\ Accuracy\end{tabular}}   & Random Pair  & {\color[HTML]{1E1E1E} 87.06±3.40}          & {\color[HTML]{1E1E1E} 87.96±3.44}          & {\color[HTML]{1E1E1E} 88.55±3.15}          & {\color[HTML]{1E1E1E} 86.64±2.98}          & 87.55±3.24                                             \\ \cline{2-8} 
                                   &                                                                                     & ImageNet     & {\color[HTML]{1E1E1E} 87.10±4.80}          & {\color[HTML]{1E1E1E} 88.06±5.11}          & {\color[HTML]{1E1E1E} 84.19±4.28}          & {\color[HTML]{1E1E1E} 85.01±5.27}          & 86.09±4.86                                             \\
                                   &                                                                                     & FixedPair    & {\color[HTML]{1E1E1E} 87.45±3.96}          & {\color[HTML]{1E1E1E} 86.38±3.12}          & {\color[HTML]{1E1E1E} 88.18±3.00}          & {\color[HTML]{1E1E1E} \textbf{88.89±2.98}} & \multicolumn{1}{l}{{\color[HTML]{444444} 87.72 ±3.27}} \\
                                   &                                                                                     & Ordered Pair & {\color[HTML]{1E1E1E} \textbf{87.88±2.89}} & {\color[HTML]{1E1E1E} \textbf{88.21±3.21}} & {\color[HTML]{1E1E1E} \textbf{89.52±3.26}} & {\color[HTML]{1E1E1E} 87.90±3.03}          & \textbf{88.38±3.09}                                    \\
\multirow{-8}{*}{ResNet-50}        & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Patient Level\\  Accuracy\end{tabular}} & Random Pair  & {\color[HTML]{1E1E1E} 87.17±2.98}          & {\color[HTML]{1E1E1E} 87.96±3.02}          & {\color[HTML]{1E1E1E} 88.76±3.55}          & {\color[HTML]{1E1E1E} 88.06±3.00}          & 87.99±3.14                         \\ \hline                    
\end{tabular}
\end{scriptsize}
\end{table*}

==> WACV 2021-MPCS_Arxiv/sections/tables/evaluation_FT80.tex <==
\begin{table}[t]
\centering
\caption{Performance evaluation in fully supervised setting when fine-tuning with 80\% labelled data (trainset).}
\label{tab:results_ft80}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Metric                                                                              & Method            & 40X                                        & 100X                                        & 200X                                       & 400X                                       & Mean                \\ \hline
                                                                                    & ImageNet & {\color[HTML]{1E1E1E} 92.12±5.32}          & {\color[HTML]{1E1E1E} 92.66±4.79}           & {\color[HTML]{1E1E1E} 91.83±7.03}          & {\color[HTML]{1E1E1E} 88.35±6.38}          & 91.24±5.88          \\
                                                                                    & MPCS-Ordered Pair      & {\color[HTML]{1E1E1E} 92.67±6.16}          & {\color[HTML]{1E1E1E} \textbf{93.63±5.31}}  & {\color[HTML]{1E1E1E} \textbf{92.72±5.95}} & {\color[HTML]{1E1E1E} 88.74±5.83}          & 91.94±5.81          \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Image Level \\ Accuracy\end{tabular}}   & MPCS-Random Pair       & {\color[HTML]{1E1E1E} \textbf{93.45±5.53}} & {\color[HTML]{1E1E1E} 93.38±4.55}           & {\color[HTML]{1E1E1E} 92.28±6.19}          & {\color[HTML]{1E1E1E} \textbf{89.81±6.05}} & \textbf{92.23±5.58} \\ \hline
                                                                                    & Transfer Learning & {\color[HTML]{1E1E1E} 91.91 ± 5.01}        & {\color[HTML]{1E1E1E} 91.93 ± 4.21}         & {\color[HTML]{1E1E1E} 91.46 ± 6.26}        & {\color[HTML]{1E1E1E} 88.10±5.07}          & 90.85±5.13          \\
                                                                                    & MPCS-Ordered Pair      & {\color[HTML]{1E1E1E} 92.45±6.65}          & {\color[HTML]{1E1E1E} 93.47±5.31}           & {\color[HTML]{1E1E1E} \textbf{92.44±4.30}} & {\color[HTML]{1E1E1E} 88.15±3.91}          & 91.63±5.04          \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Patient Level\\  Accuracy\end{tabular}} & MPCS-Random Pair       & {\color[HTML]{1E1E1E} \textbf{93.26±5.4}}  & {\color[HTML]{1E1E1E} \textbf{93.57± 4.36}} & {\color[HTML]{1E1E1E} 92.23±6.01}          & {\color[HTML]{1E1E1E} \textbf{89.57±3.79}} & \textbf{92.15±4.89} \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/evaluation_comparision.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\caption{Comparison of proposed methods with state-of-the-art methods on downstream task of classifying histopathological images at different magnification factors in fully supervised setting(using 100\% train set labels). RN-50 indicates ResNet-50 and Eff-net b2 indicates Efficient-net b2 encoder. Also, OP indicates Ordered Pair, FP indicates Fixed Pair, and RP indcates Random Pair.}
\label{ft_80_sota}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|cccc|c|cccc|c}

\hline
                                                            & \multicolumn{4}{c|}{Patient Level Accuracy (RR)}                                                                                                                                                                           &                        & \multicolumn{4}{c|}{Image Level Accuracy}                                                                                                            &                                                       \\ \cline{2-5} \cline{7-10}
\multirow{-2}{*}{Method}                                    & \multicolumn{1}{c|}{40X}                 & \multicolumn{1}{c|}{100X}                                        & \multicolumn{1}{c|}{200X}                                       & 400X                                       & \multirow{-2}{*}{Mean} & \multicolumn{1}{c|}{40X}                 & \multicolumn{1}{c|}{100X}                & \multicolumn{1}{c|}{200X}                & 400X                & \multirow{-2}{*}{Mean}                                \\
\hline
Original-GLCM\cite{spanhol2016breast}   & \multicolumn{1}{c|}{74.7±1.0}            & \multicolumn{1}{c|}{78.6±2.6}                                    & \multicolumn{1}{c|}{83.4±3.3}                                   & 81.7±3.3                                   & 79.60±2.55             & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & -                   & -                                                     \\
PFTAS\cite{hamilton2007fast}               & \multicolumn{1}{c|}{83.80±2.0}           & \multicolumn{1}{c|}{82.10±4.9}                                   & \multicolumn{1}{c|}{85.10±3.1}                                  & 82.30±3.8                                  & 83.33±3.45             & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & -                   & -                                                     \\
MIL-NP\cite{sudharshan2019multiple}        & \multicolumn{1}{c|}{92.1±5.9}            & \multicolumn{1}{c|}{89.1±5.2}                                    & \multicolumn{1}{c|}{87.2±4.3}                                   & 82.7±3.0                                   & 87.77±4.6              & \multicolumn{1}{c|}{87.8±5.6}            & \multicolumn{1}{c|}{85.6±4.3}            & \multicolumn{1}{c|}{80.8±2.8}            & 82.9±4.1            & \multicolumn{1}{l}{{\color[HTML]{444444} 84.28±4.20}} \\
SW\cite{spanhol2016breast}                 & \multicolumn{1}{c|}{88.6±5.6}            & \multicolumn{1}{c|}{84.5±2.4}                                    & \multicolumn{1}{c|}{85.3±3.8}                                   & 81.7±4.9                                   & 85.02±4.17             & \multicolumn{1}{c|}{89.6±6.58}           & \multicolumn{1}{c|}{85.0±4.8}            & \multicolumn{1}{c|}{84.0±3.2}            & 80.8±3.1            & \multicolumn{1}{l}{{\color[HTML]{444444} 84.85±4.42}} \\
MI\cite{bayramoglu2016deep}                & \multicolumn{1}{c|}{83.08±2.08}          & \multicolumn{1}{c|}{83.17±3.51}                                  & \multicolumn{1}{c|}{84.63±2.72}                                 & 82.10±4.42                                 & 83.25±3.18             & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & -                   & -                                                     \\
Deep\cite{spanhol2017deep}                 & \multicolumn{1}{c|}{84.0±6.9}            & \multicolumn{1}{c|}{83.9±5.9}                                    & \multicolumn{1}{c|}{86.3±3.5}                                   & 82.1±2.4                                   & 84.07±4.67             & \multicolumn{1}{c|}{84.6±2.9}            & \multicolumn{1}{c|}{84.8±4.2}            & \multicolumn{1}{c|}{84.2±1.7}            & 81.6±3.7            & \multicolumn{1}{l}{{\color[HTML]{444444} 83.80±3.13}} \\
MILCNN\cite{sudharshan2019multiple}        & \multicolumn{1}{c|}{86.9±5.4}            & \multicolumn{1}{c|}{85.7±4.8}                                    & \multicolumn{1}{c|}{85.9±3.9}                                   & 83.4±5.3                                   & 85.47±4.85             & \multicolumn{1}{c|}{86.1 ± 4.28}         & \multicolumn{1}{c|}{83.8±3.0}            & \multicolumn{1}{c|}{80.2±2.6}            & 80.6±4.6            & \multicolumn{1}{l}{{\color[HTML]{444444} 82.68±3.62}} \\
GLPB\cite{ataky2020data}                   & \multicolumn{1}{c|}{84.5±4.2}            & \multicolumn{1}{c|}{83.5±2.0}                                    & \multicolumn{1}{c|}{89.6±5.0}                                   & \textbf{88.2±4.0}                          & 86.45±3.8              & \multicolumn{1}{c|}{82.1±6.4}            & \multicolumn{1}{c|}{81.4±4.8}            & \multicolumn{1}{c|}{88.4±5.0}            & 87.2±4.5            & \multicolumn{1}{l}{{\color[HTML]{444444} 84.78±5.18}} \\
RPDB\cite{man2020classification}$^\Cross$  & \multicolumn{1}{c|}{92.02±0.9}           & \multicolumn{1}{c|}{90.21±2.40}                                  & \multicolumn{1}{c|}{81.94±1.70}                                 & 80.09±0.70                                 & 88.06±1.4              & \multicolumn{1}{c|}{\textbf{94.26±3.2}}  & \multicolumn{1}{c|}{92.71±0.4}           & \multicolumn{1}{c|}{83.90±2.8}           & 82.74±1.5           & \multicolumn{1}{l}{{\color[HTML]{444444} 88.40±1.98}} \\
SMSE\cite{sun2021magnificationindependent} & \multicolumn{1}{c|}{87.51±4.07}          & \multicolumn{1}{c|}{89.12±2.86}                                  & \multicolumn{1}{c|}{90.83±3.31}                                 & 87.10±3.80                                 & 88.64±3.51             & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & \multicolumn{1}{c|}{-}                   & -                   & -                                                     \\ \hline
ImageNet (Eff-net b2)                                       & \multicolumn{1}{c|}{91.91±4.25}          & \multicolumn{1}{c|}{91.93±4.20}                                  & \multicolumn{1}{c|}{91.46±5.17}                                 & 88.10±3.88                                 & 90.85±4.36             & \multicolumn{1}{c|}{92.12±4.18}          & \multicolumn{1}{c|}{92.66±4.20}          & \multicolumn{1}{c|}{91.83±4.55}          & 88.35±5.21          & 91.24±4.54                                            \\
MPCS-FP (Eff-net b2)                                        & \multicolumn{1}{c|}{92.23±3.50}          & \multicolumn{1}{c|}{92.72±3.68}                                  & \multicolumn{1}{c|}{91.94±3.80}                                 & 88.40±3.26                                 & 91.33±3.56             & \multicolumn{1}{c|}{92.23±3.80}          & \multicolumn{1}{c|}{\textbf{93.57±3.23}} & \multicolumn{1}{c|}{92.23±2.98}          & 88.40±3.90          & 91.61±3.48                                            \\
MPCS-OP (Eff-net b2)                                        & \multicolumn{1}{c|}{\textbf{92.45±3.25}} & \multicolumn{1}{c|}{\textbf{93.47±2.98}}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{92.44±3.30}}} & {\color[HTML]{1E1E1E} 89.00±3.05}          & \textbf{91.84±3.15}    & \multicolumn{1}{c|}{92.67±3.36}          & \multicolumn{1}{c|}{\textbf{93.63±3.38}} & \multicolumn{1}{c|}{\textbf{92.72±2.80}} & \textbf{88.74±3.90} & \textbf{91.94±3.36}                                   \\
MPCS-RP (Eff-net b2)                                        & \multicolumn{1}{c|}{\textbf{93.26±3.48}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{93.57± 3.36}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{92.23±3.21}}} & {\color[HTML]{1E1E1E} \textbf{89.57±3.79}} & \textbf{92.15±3.46}    & \multicolumn{1}{c|}{\textbf{93.45±3.55}} & \multicolumn{1}{c|}{93.38±2.80}          & \multicolumn{1}{c|}{\textbf{92.28±3.49}} & \textbf{89.81±3.15} & \textbf{92.23±3.24}                                   \\
ImageNet (RN-50)                                            & \multicolumn{1}{c|}{91.46±4.30}          & \multicolumn{1}{c|}{91.24±5.1}                                   & \multicolumn{1}{c|}{90.72±4.68}                                 & 87.90±4.12                                 & 90.33±4.55             & \multicolumn{1}{c|}{91.83±5.12}          & \multicolumn{1}{c|}{92.23±4.15}          & \multicolumn{1}{c|}{91.61±4.00}          & 87.88±4.80          & 90.89±4.52                                            \\
MPCS-FP (RN-50)                                             & \multicolumn{1}{c|}{91.83±3.88}          & \multicolumn{1}{c|}{92.67±2.72}                                  & \multicolumn{1}{c|}{91.61±3.40}                                 & 89.00±3.15                                 & 91.28±3.29             & \multicolumn{1}{c|}{92.24±3.48}          & \multicolumn{1}{c|}{92.66±3.88}          & \multicolumn{1}{c|}{91.91±3.68}          & 88.40±3.66          & 91.30±3.68                                            \\
MPCS-OP (RN-50)                                             & \multicolumn{1}{c|}{\textbf{93.00±3.66}} & \multicolumn{1}{c|}{93.26±3.08}                                  & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{92.28±2.88}}} & {\color[HTML]{1E1E1E} \textbf{88.74±3.60}} & \textbf{91.82±3.31}    & \multicolumn{1}{c|}{\textbf{93.26±3.40}} & \multicolumn{1}{c|}{\textbf{93.45±2.89}} & \multicolumn{1}{c|}{\textbf{92.45±3.77}} & \textbf{89.57±2.96} & \textbf{92.18±3.26}                                   \\
MPCS-RP (RN-50)                                             & \multicolumn{1}{c|}{92.72±3.50}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{93.57± 2.88}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 92.23±3.90}}          & {\color[HTML]{1E1E1E} 88.40±3.05}          & 91.73±3.33             & \multicolumn{1}{c|}{92.72±3.38}          & \multicolumn{1}{c|}{92.72±4.02}          & \multicolumn{1}{c|}{91.91±3.21}          & 88.56±3.89          & 91.48±3.66                                            \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}


==> WACV 2021-MPCS_Arxiv/sections/tables/exp_stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\caption{Experimentation statistics for proposed method MPCS}
\label{tab:exp_stats}
%\resizebox{\columnwidth}{!}{%
%\resizebox{\columnwidth}{!}{%
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|c}
\hline
\multicolumn{1}{c|}{Dataset}                    & Experiment Training Type          & No. of Experiments         \\ \hline
\multicolumn{1}{c|}{}                           & SSL pretrain - Efficient-net b2   & 15                         \\
\multicolumn{1}{c|}{}                           & SSL pretrain - ResNet-50          & 18                         \\
\multicolumn{1}{c|}{}                           & Downstream task- Efficient-net b2 & 400                        \\
\multicolumn{1}{c|}{\multirow{-4}{*}{BreakHis}} & Downstream task- ResNet-50        & {\color[HTML]{1E1E1E} 400} \\ \hline
\multicolumn{1}{c|}{BACH}                       & Downstream task- ResNet-50        & 140                        \\ \hline
\multicolumn{1}{c|}{Breast Cell Cancer Dataset} & Downstream task- ResNet-50        & 30                         \\ \hline
\multicolumn{2}{c|}{\textbf{Total}}                                                 & \textbf{1003}              \\ \hline
\end{tabular} 
\end{table*}

==> WACV 2021-MPCS_Arxiv/sections/tables/mpcs_breakhis_on_40_labels_of_trainset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h!t]
\centering
\caption{Performance evaluation of the proposed methods in limited labelled data setting when fine-tuning on 40\% labels of train set.}
\label{tab:breakhis_40_label_mpcs}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|cccc|c|cccc|c}
\hline
                         & \multicolumn{4}{c|}{Patient Level Accuracy (RR)}                                                                                                                                       &                        & \multicolumn{4}{c|}{Image Level Accuracy}                                                                        &                        \\ \cline{2-5} \cline{7-10}
\multirow{-2}{*}{Method} & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}                               & \multicolumn{1}{c|}{200X}                              & 400X                              & \multirow{-2}{*}{Mean} & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}       & \multicolumn{1}{c|}{200X}       & 400X       & \multirow{-2}{*}{Mean} \\ \hline
ImageNet (Eff-net b2)    & \multicolumn{1}{c|}{87.45±3.04} & \multicolumn{1}{c|}{88.00±3.22}                         & \multicolumn{1}{c|}{87.52±3.56}                        & 85.95±3.11                        & 87.03±3.23             & \multicolumn{1}{c|}{88.05±3.11} & \multicolumn{1}{c|}{89.14±3.22} & \multicolumn{1}{c|}{88.00±3.19} & 85.02±3.00 & 87.55±3.13             \\
MPCS-FP (Eff-net b2)     & \multicolumn{1}{c|}{88.66±3.62} & \multicolumn{1}{c|}{88.90±3.10}                         & \multicolumn{1}{c|}{89.66±2.03}                        & 88.30±3.12                        & 88.88±2.98             & \multicolumn{1}{c|}{88.02±3.72} & \multicolumn{1}{c|}{89.28±3.04} & \multicolumn{1}{c|}{90.00±2.16} & 88.15±3.06 & 88.86±3.00             \\
MPCS-OP (Eff-net b2)     & \multicolumn{1}{c|}{89.75±3.56} & \multicolumn{1}{c|}{90.63±2.66}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.32±3.11}} & {\color[HTML]{1E1E1E} 88.96±3.55} & 89.92±3.22             & \multicolumn{1}{c|}{88.82±3.22} & \multicolumn{1}{c|}{90.04±2.89} & \multicolumn{1}{c|}{90.60±3.43} & 88.40±3.89 & 89.47±3.36             \\
MPCS-RP (Eff-net b2)     & \multicolumn{1}{c|}{89.05±3.27} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.05± 3.42}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 89.80±2.82}} & {\color[HTML]{1E1E1E} 88.70±2.65} & 89.40±3.04             & \multicolumn{1}{c|}{90.25±3.21} & \multicolumn{1}{c|}{91.00±3.36} & \multicolumn{1}{c|}{90.05±3.11} & 87.40±3.45 & 89.70±2.53             \\
ImageNet (RN-50)         & \multicolumn{1}{c|}{88.01±3.65} & \multicolumn{1}{c|}{88.50±3.43}                         & \multicolumn{1}{c|}{87.09±3.62}                        & 85.88±3.01                        & 87.37±3.43             & \multicolumn{1}{c|}{88.10±3.23} & \multicolumn{1}{c|}{88.60±3.53} & \multicolumn{1}{c|}{88.02±3.00} & 85.60±3.22 & 87.78±3.25             \\
MPCS-FP (RN-50)          & \multicolumn{1}{c|}{88.20±3.61} & \multicolumn{1}{c|}{88.17±2.62}                         & \multicolumn{1}{c|}{89.00±3.81}                        & 88.90±3.56                        & 88.58±3.4              & \multicolumn{1}{c|}{87.90±3.25} & \multicolumn{1}{c|}{88.10±3.21} & \multicolumn{1}{c|}{88.50±3.61} & 88.10±3.56 & 88.15±3.41             \\
MPCS-OP (RN-50)          & \multicolumn{1}{c|}{89.42±2.13} & \multicolumn{1}{c|}{90.28±3.64}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 89.92±2.18}} & {\color[HTML]{1E1E1E} 88.02±3.22} & 89.41±2.79             & \multicolumn{1}{c|}{89.10±3.05} & \multicolumn{1}{c|}{90.00±2.85} & \multicolumn{1}{c|}{89.90±2.52} & 87.80±2.65 & 89.20±2.78             \\
MPCS-RP (RN-50)          & \multicolumn{1}{c|}{89.01±3.32} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 89.10± 3.82}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.00±3.46}} & {\color[HTML]{1E1E1E} 88.15±3.26} & 89.06±3.47             & \multicolumn{1}{c|}{88.10±2.35} & \multicolumn{1}{c|}{89.30±3.20} & \multicolumn{1}{c|}{88.90±3.05} & 86.85±3.22 & 88.29±2.96             \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> WACV 2021-MPCS_Arxiv/sections/tables/mpcs_breakhis_on_60_labels_of_trainset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\caption{Performance evaluation of the proposed methods in limited labelled data setting when fine-tuning on 60\% labels of train set.}
\label{tab:breakhis_60_label_mpcs}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|cccc|c|cccc|c}
\hline
                         & \multicolumn{4}{c|}{Patient Level Accuracy (RR)}                                                                                                                                       &                                   & \multicolumn{4}{c|}{Image Level Accuracy}                                                                        &                        \\ \cline{2-5} \cline{7-10}
\multirow{-2}{*}{Method} & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}                               & \multicolumn{1}{c|}{200X}                              & 400X                              & \multirow{-2}{*}{Mean}            & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}       & \multicolumn{1}{c|}{200X}       & 400X       & \multirow{-2}{*}{Mean} \\ \hline
ImageNet (Eff-net b2)    & \multicolumn{1}{c|}{89.28±3.56} & \multicolumn{1}{c|}{89.03±3.40}                         & \multicolumn{1}{c|}{89.22±3.12}                        & 86.10±3.32                        & 88.40±3.35                        & \multicolumn{1}{c|}{90.02±3.54} & \multicolumn{1}{c|}{90.16±3.53} & \multicolumn{1}{c|}{89.11±3.21} & 86.00±3.52 & 88.82±3.45             \\
MPCS-FP (Eff-net b2)     & \multicolumn{1}{c|}{90.22±3.87} & \multicolumn{1}{c|}{90.45±3.20}                         & \multicolumn{1}{c|}{89.72±2.70}                        & 88.32±3.21                        & 89.67±3.25                        & \multicolumn{1}{c|}{90.56±3.32} & \multicolumn{1}{c|}{91.28±3.43} & \multicolumn{1}{c|}{90.20±2.55} & 88.20±3.40 & 90.06±3.30             \\
MPCS-OP (Eff-net b2)     & \multicolumn{1}{c|}{91.10±3.21} & \multicolumn{1}{c|}{91.54±2.66}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.44±2.65}} & {\color[HTML]{1E1E1E} 88.96±3.55} & 90.51±3.02                        & \multicolumn{1}{c|}{90.50±3.22} & \multicolumn{1}{c|}{91.74±2.66} & \multicolumn{1}{c|}{90.63±3.41} & 88.49±3.91 & 90.34±3.30             \\
MPCS-RP (Eff-net b2)     & \multicolumn{1}{c|}{91.00±4.18} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.30± 3.22}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.10±2.61}} & {\color[HTML]{1E1E1E} 89.00±2.55} & 90.10±3.14                        & \multicolumn{1}{c|}{91.15±3.43} & \multicolumn{1}{c|}{91.26±3.11} & \multicolumn{1}{c|}{91.01±3.26} & 87.53±3.02 & 90.23±3.21             \\
ImageNet (RN-50)         & \multicolumn{1}{c|}{88.90±3.44} & \multicolumn{1}{c|}{89.05±3.3}                          & \multicolumn{1}{c|}{88.04±3.23}                        & 86.04±3.24                        & 88.00±3.30                        & \multicolumn{1}{c|}{89.01±4.10} & \multicolumn{1}{c|}{89.65±3.55} & \multicolumn{1}{c|}{89.02±3.44} & 86.00±3.12 & 88.42±3.55             \\
MPCS-FP (RN-50)          & \multicolumn{1}{c|}{89.23±3.21} & \multicolumn{1}{c|}{90.11±2.32}                         & \multicolumn{1}{c|}{89.30±3.12}                        & 88.90±3.15                        & 89.39±2.95                        & \multicolumn{1}{c|}{89.05±3.33} & \multicolumn{1}{c|}{90.05±3.55} & \multicolumn{1}{c|}{89.56±3.65} & 88.21±3.56 & 89.21±3.52             \\
MPCS-OP (RN-50)          & \multicolumn{1}{c|}{91.02±2.54} & \multicolumn{1}{c|}{91.08±3.18}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.05±2.78}} & {\color[HTML]{1E1E1E} 88.21±3.22} & {\color[HTML]{1E1E1E} 90.09±3.22} & \multicolumn{1}{c|}{91.05±3.66} & \multicolumn{1}{c|}{91.01±2.70} & \multicolumn{1}{c|}{90.10±2.32} & 88.00±2.60 & 90.04±2.82             \\
MPCS-RP (RN-50)          & \multicolumn{1}{c|}{90.01±3.22} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.10± 3.28}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 90.21±3.56}} & {\color[HTML]{1E1E1E} 88.22±3.20} & 89.64±3.32                        & \multicolumn{1}{c|}{90.05±2.32} & \multicolumn{1}{c|}{90.02±3.16} & \multicolumn{1}{c|}{89.01±3.55} & 86.90±3.21 & 89.00±3.06             \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> WACV 2021-MPCS_Arxiv/sections/tables/mpcs_breakhis_on_80_labels_of_trainset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\caption{Performance evaluation of the proposed methods in limited labelled data setting when fine-tuning on 80\% labels of train set.}
\label{tab:breakhis_80_label_mpcs}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|cccc|c|cccc|c}
\hline
                         & \multicolumn{4}{c|}{Patient Level Accuracy (RR)}                                                                                                                                       &                        & \multicolumn{4}{c|}{Image Level Accuracy}                                                                        &                        \\ \cline{2-5} \cline{7-10}
\multirow{-2}{*}{Method} & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}                               & \multicolumn{1}{c|}{200X}                              & 400X                              & \multirow{-2}{*}{Mean} & \multicolumn{1}{c|}{40X}        & \multicolumn{1}{c|}{100X}       & \multicolumn{1}{c|}{200X}       & 400X       & \multirow{-2}{*}{Mean} \\ \hline
ImageNet (Eff-net b2)    & \multicolumn{1}{c|}{90.48±3.45} & \multicolumn{1}{c|}{90.53±3.60}                         & \multicolumn{1}{c|}{90.36±4.67}                        & 87.30±3.88                        & 89.66±3.90             & \multicolumn{1}{c|}{91.32±3.48} & \multicolumn{1}{c|}{91.46±3.40} & \multicolumn{1}{c|}{90.34±3.55} & 87.32±4.76 & 90.11±3.79             \\
MPCS-FP (Eff-net b2)     & \multicolumn{1}{c|}{91.26±3.64} & \multicolumn{1}{c|}{91.54±3.68}                         & \multicolumn{1}{c|}{90.84±2.66}                        & 88.32±3.23                        & 90.49±3.30             & \multicolumn{1}{c|}{91.83±3.48} & \multicolumn{1}{c|}{92.34±3.20} & \multicolumn{1}{c|}{91.33±2.45} & 88.30±3.50 & 90.95±3.15             \\
MPCS-OP (Eff-net b2)     & \multicolumn{1}{c|}{92.05±3.17} & \multicolumn{1}{c|}{92.73±2.45}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.54±2.80}} & {\color[HTML]{1E1E1E} 88.98±3.42} & 91.33±2.96             & \multicolumn{1}{c|}{91.67±3.53} & \multicolumn{1}{c|}{92.45±2.80} & \multicolumn{1}{c|}{91.45±3.60} & 88.55±3.40 & 91.03±3.33             \\
MPCS-RP (Eff-net b2)     & \multicolumn{1}{c|}{92.16±4.18} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.51± 3.18}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.13±2.81}} & {\color[HTML]{1E1E1E} 89.16±2.43} & 91.00±3.15             & \multicolumn{1}{c|}{92.25±3.61} & \multicolumn{1}{c|}{92.48±3.20} & \multicolumn{1}{c|}{92.01±3.49} & 88.71±3.15 & 91.36±3.79             \\
ImageNet (RN-50)         & \multicolumn{1}{c|}{90.16±3.40} & \multicolumn{1}{c|}{90.01±4.1}                          & \multicolumn{1}{c|}{89.32±3.54}                        & 87.00±4.45                        & 89.12±3.87             & \multicolumn{1}{c|}{90.53±5.12} & \multicolumn{1}{c|}{91.03±3.23} & \multicolumn{1}{c|}{90.31±3.59} & 86.48±4.92 & 89.58±4.21             \\
MPCS-FP (RN-50)          & \multicolumn{1}{c|}{90.44±3.43} & \multicolumn{1}{c|}{91.32±2.54}                         & \multicolumn{1}{c|}{90.43±3.32}                        & 88.95±2.10                        & 90.29±2.85             & \multicolumn{1}{c|}{90.14±3.48} & \multicolumn{1}{c|}{91.00±3.88} & \multicolumn{1}{c|}{90.71±3.24} & 88.30±2.46 & 90.04±3.27             \\
MPCS-OP (RN-50)          & \multicolumn{1}{c|}{92.00±2.42} & \multicolumn{1}{c|}{92.16±3.08}                         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.15±2.88}} & {\color[HTML]{1E1E1E} 88.30±3.30} & 90.90±2.92             & \multicolumn{1}{c|}{92.16±2.80} & \multicolumn{1}{c|}{92.15±2.89} & \multicolumn{1}{c|}{91.05±2.43} & 88.50±2.45 & 90.00±2.64             \\
MPCS-RP (RN-50)          & \multicolumn{1}{c|}{91.02±3.56} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.20± 3.28}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 91.10±3.88}} & {\color[HTML]{1E1E1E} 88.20±3.17} & 90.38±2.92             & \multicolumn{1}{c|}{91.02±2.44} & \multicolumn{1}{c|}{91.22±3.13} & \multicolumn{1}{c|}{90.02±3.65} & 87.06±3.84 & 89.80±3.27             \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> WACV 2021-MPCS_Arxiv/sections/tables/tab_bach_experiments.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{Experiment details for BACH datasets}
\label{tab:exp_bach}
\begin{tabular}{c|c|cc}
\hline
                      &                                                                                          & \multicolumn{2}{c}{Fine-tuning on BACH dataset}                                                                   \\ \cline{3-4} 
\multirow{-2}{*}{No.} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-training \\ method/weights\end{tabular}} & \multicolumn{1}{c|}{Train data(\%)}                                                 & Test data (\%)              \\ \hline
Exp-9                 & ImageNet                                                                                 & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}                                    & {\color[HTML]{1E1E1E} 20\%} \\
Exp-10                & MPCS-Fixed Pair (BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\
Exp-11                & MPCS-Ordered Pair(BreakHis)                                                              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & 20\%                        \\
Exp-12                & MPCS-Random Pair(BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\ \hline
\end{tabular}
\end{table}

==> WACV 2021-MPCS_Arxiv/sections/tables/trained_cross_magnification.tex <==
\begin{table}[h]
\caption{Type 1 cross magnification performance  comparison of proposed methods (Leave one magnification out on which model trained). The values represent mean performance of remaining magnifications (e.g. train on 40x and evaluated (mean) on 100x, 200x, and 400x.)}
%\caption{Comparison of Proposed self-supervised pre-training methods MPCS-Ordered Pair \& MPCS-Random Pair with (ImageNet pretrained) Transfer Learning on mean cross-magnification performance (excludes magnification on which model trained) in fully supervised setting}
\label{tab:results_ft80_cross_magnificaiton}
\resizebox{\columnwidth}{!}{%

\begin{tabular}{c|cccc}
\hline
                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Trained \\ on 40X\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Trained \\ on 100X\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Trained \\ on 200X\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Trained \\ on 400X\end{tabular}     \\ \cline{2-5} 
\multirow{-2}{*}{Method} & \multicolumn{4}{c}{Mean Cross-Magnification Image Level Accuracy}                                                                                                                                                                                                                                                   \\ \hline
ImageNet        & \multicolumn{1}{l|}{{\color[HTML]{444444} 79.56±11.74}}                        & \multicolumn{1}{l|}{{\color[HTML]{444444} 79.56±11.74}}                         & \multicolumn{1}{l|}{{\color[HTML]{444444} 82.97±6.77}}                          & \multicolumn{1}{l}{{\color[HTML]{444444} 84.16±4.98}}          \\
MPCS-Ordered Pair             & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{80.99±8.91}}}                & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{80.99±8.91}}}                 & \multicolumn{1}{l|}{{\color[HTML]{444444} 84.40±3.81}}                          & \multicolumn{1}{l}{{\color[HTML]{444444} 84.20±5.58}}          \\
MPCS-Random Pair              & \multicolumn{1}{l|}{{\color[HTML]{444444} 80.13±9.60}}                         & \multicolumn{1}{l|}{{\color[HTML]{444444} 80.13±9.60}}                          & \multicolumn{1}{l|}{{\color[HTML]{444444} \textbf{84.84±5.30}}}                 & \multicolumn{1}{l}{{\color[HTML]{444444} \textbf{84.83±5.30}}} \\ \hline
\multicolumn{1}{l|}{}    & \multicolumn{4}{c}{Mean Cross-Magnification Patient Level Accuracy}                                                                                                                                                                                                                                                 \\ \hline
ImageNet        & \multicolumn{1}{c|}{{\color[HTML]{444444} 81.01±9.59}}                         & \multicolumn{1}{c|}{{\color[HTML]{444444} 84.38±5.78}}                          & \multicolumn{1}{c|}{{\color[HTML]{444444} 81.45±6.89}}                          & {\color[HTML]{444444} 83.31±7.31}                              \\
MPCS-Ordered Pair             & \multicolumn{1}{c|}{{\color[HTML]{444444} \textbf{81.49±6.96}}}                & \multicolumn{1}{c|}{{\color[HTML]{444444} 84.02±5.78}}                          & \multicolumn{1}{c|}{{\color[HTML]{444444} 82.19±3.83}}                          & {\color[HTML]{444444} 83.10±7.44}                              \\
MPCS-Random Pair              & \multicolumn{1}{c|}{{\color[HTML]{444444} 81.20±7.09}}                         & \multicolumn{1}{c|}{{\color[HTML]{444444} \textbf{85.05±7.15}}}                 & \multicolumn{1}{c|}{{\color[HTML]{444444} \textbf{82.97±5.84}}}                 & {\color[HTML]{444444} \textbf{83.76±6.63}}                     \\ \hline
\end{tabular}%
}
\label{x_mag_type1}
%\vspace{-3mm}
\end{table}

==> sections/4_dataset.tex <==
The BreaKHis dataset~\cite{spanhol2016dataset} contains 7909 microscopic histopathology whole slide images (WSI) categorized into benign and malignant classes of breast tumor. WSI is collected from 82 patients, 24 benign and 58 malignant. Images of each patient are provided in four different magnifications 40x, 100x, 200x, and 400x respectively, and their detailed description is mentioned in Table~\ref{tab:experiments_details}. Evaluation metrics suggested in BreakHis~\cite{spanhol2016dataset} and followed by many state-of-the-art methods are \textit{Image-Level Accuracy (ILA)} and \textit{Patient-Level Accuracy (PLA)}. ILA corresponds to the score from the total number of correctly classified images. PLA, also called \textit{Recognition Rate} corresponds to the average image-level accuracy per patient.
This work follows the same evaluation scheme.
Additionally, the cross-magnification evaluation is also performed using both evaluation metrics.


\begin{table}[t]
\caption{Description of BreakHis dataset.}
\label{tab:BreakHis_dataset}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc|c|c}
\hline
                           & \multicolumn{4}{c|}{Magnification}                                                                                                                                                                                       &                         &                           \\
\multirow{-2}{*}{Category} & \multicolumn{1}{c|}{\textbf{40X}}                         & \multicolumn{1}{c|}{\textbf{100X}}                        & \multicolumn{1}{c|}{\textbf{200X}}                        & \textbf{400X}                        & \multirow{-2}{*}{Total} & \multirow{-2}{*}{Patient} \\ \hline
\textbf{Benign}            & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 625}}           & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 644}}           & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 623}}           & {\color[HTML]{1E1E1E} 588}           & 2480                    & 24                        \\
\textbf{Malignant}         & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1370}}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1437}}          & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 1390}}          & {\color[HTML]{1E1E1E} 1232}          & 5429                    & {\color[HTML]{444444} 58} \\ \hline
\textbf{Total}             & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{1995}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{2081}}} & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} \textbf{2013}}} & {\color[HTML]{1E1E1E} \textbf{1820}} & \textbf{7909}           & \textbf{82}               \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}

==> sections/tables/evaluation_FT80.tex <==
\begin{table}[t]
\centering
\caption{Performance evaluation in fully supervised setting when fine-tuning with 80\% labelled data (trainset).}
\label{tab:results_ft80}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Metric                                                                              & Method            & 40X                                        & 100X                                        & 200X                                       & 400X                                       & Mean                \\ \hline
                                                                                    & ImageNet & {\color[HTML]{1E1E1E} 92.12±5.32}          & {\color[HTML]{1E1E1E} 92.66±4.79}           & {\color[HTML]{1E1E1E} 91.83±7.03}          & {\color[HTML]{1E1E1E} 88.35±6.38}          & 91.24±5.88          \\
                                                                                    & MPCS-Ordered Pair      & {\color[HTML]{1E1E1E} 92.67±6.16}          & {\color[HTML]{1E1E1E} \textbf{93.63±5.31}}  & {\color[HTML]{1E1E1E} \textbf{92.72±5.95}} & {\color[HTML]{1E1E1E} 88.74±5.83}          & 91.94±5.81          \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Image Level \\ Accuracy\end{tabular}}   & MPCS-Random Pair       & {\color[HTML]{1E1E1E} \textbf{93.45±5.53}} & {\color[HTML]{1E1E1E} 93.38±4.55}           & {\color[HTML]{1E1E1E} 92.28±6.19}          & {\color[HTML]{1E1E1E} \textbf{89.81±6.05}} & \textbf{92.23±5.58} \\ \hline
                                                                                    & Transfer Learning & {\color[HTML]{1E1E1E} 91.91 ± 5.01}        & {\color[HTML]{1E1E1E} 91.93 ± 4.21}         & {\color[HTML]{1E1E1E} 91.46 ± 6.26}        & {\color[HTML]{1E1E1E} 88.10±5.07}          & 90.85±5.13          \\
                                                                                    & MPCS-Ordered Pair      & {\color[HTML]{1E1E1E} 92.45±6.65}          & {\color[HTML]{1E1E1E} 93.47±5.31}           & {\color[HTML]{1E1E1E} \textbf{92.44±4.30}} & {\color[HTML]{1E1E1E} 88.15±3.91}          & 91.63±5.04          \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Patient Level\\  Accuracy\end{tabular}} & MPCS-Random Pair       & {\color[HTML]{1E1E1E} \textbf{93.26±5.4}}  & {\color[HTML]{1E1E1E} \textbf{93.57± 4.36}} & {\color[HTML]{1E1E1E} 92.23±6.01}          & {\color[HTML]{1E1E1E} \textbf{89.57±3.79}} & \textbf{92.15±4.89} \\ \hline
\end{tabular}%
}
\vspace{-6mm}
\end{table}

==> sections/tables/tab_bach_experiments.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{Experiment details for BACH datasets}
\label{tab:exp_bach}
\begin{tabular}{c|c|cc}
\hline
                      &                                                                                          & \multicolumn{2}{c}{Fine-tuning on BACH dataset}                                                                   \\ \cline{3-4} 
\multirow{-2}{*}{No.} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-training \\ method/weights\end{tabular}} & \multicolumn{1}{c|}{Train data(\%)}                                                 & Test data (\%)              \\ \hline
Exp-9                 & ImageNet                                                                                 & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} 80\%}}                                    & {\color[HTML]{1E1E1E} 20\%} \\
Exp-10                & MPCS-Fixed Pair (BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\
Exp-11                & MPCS-Ordered Pair(BreakHis)                                                              & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & 20\%                        \\
Exp-12                & MPCS-Random Pair(BreakHis)                                                               & \multicolumn{1}{c|}{{\color[HTML]{1E1E1E} {[}5\%, 10\%, 20\%, 40\%, 60\%, 80\%{]}}} & {\color[HTML]{1E1E1E} 20\%} \\ \hline
\end{tabular}
\end{table}
